NWR: Rethinking Thomas Write Rule for Omittable Write Operations

Concurrency control protocols are the key to scaling current DBMS performances. They efficiently interleave read and write operations in transactions, but occasionally they restrict concurrency by using coordination such as exclusive lockings. Although exclusive lockings ensure the correctness of DBMS, it incurs serious performance penalties on multi-core environments. In particular, existing protocols generally suffer from emerging highly write contended workloads, since they use innumerable lockings for write operations. In this paper, we rethink the Thomas write rule (TWR), which allows the timestamp ordering (T/O) protocol to omit write operations without any lockings. We formalize the notion of omitting and decouple it from the T/O protocol implementation, in order to define a new rule named non-visible write rule (NWR). When the rules of NWR are satisfied, any protocol can in theory generate omittable write operations with preserving the correctness without any lockings. In the experiments, we implement three NWR-extended protocols: Silo+NWR, TicToc+NWR, and MVTO+NWR. Experimental results demonstrate the efficiency and the low-overhead property of the extended protocols. We confirm that NWR-extended protocols achieve more than 11x faster than the originals in the best case of highly write contended YCSB-A and comparable performance with the originals in the other workloads.

==> IWR-paper copy/tex/abstract.tex <==
Concurrency control protocols are the key to scaling current DBMS performances.
They efficiently interleave read and write operations in transactions, but occasionally they restrict concurrency by using coordination such as exclusive lockings.
Although exclusive lockings ensure the correctness of DBMS, it incurs serious performance penalties on multi-core environments.
In particular, existing protocols generally suffer from emerging highly write contended workloads, since they use innumerable lockings for write operations.
In this paper, we rethink the Thomas write rule (TWR), which allows the timestamp ordering (T/O) protocol to omit write operations without any lockings.
We formalize the notion of omitting and decouple it from the T/O protocol implementation, in order to define a new rule named non-visible write rule (NWR).
When the rules of NWR are satisfied, any protocol can in theory generate omittable write operations with preserving the correctness without any lockings.
In the experiments, we implement three NWR-extended protocols: Silo+NWR, TicToc+NWR, and MVTO+NWR.
Experimental results demonstrate the efficiency and the low-overhead property of the extended protocols.
We confirm that NWR-extended protocols achieve more than 11x faster than the originals in the best case of highly write contended YCSB-A and comparable performance with the originals in the other workloads.


==> IWR-paper copy/tex/algorithms.tex <==
\section{Implementation Overview}
\label{sec:implementation_overview}

Next, we show an implementation overview of NWR.
To extend a baseline protocol to a new NWR-extended protocol, we must add followings procedures:

\begin{enumerate}
  \item
         Find and generate an additional version order $\ll^{NWR}$ which satisfies preserving version order rule
  \item
        Collect $successors_j$ and $overwriters_j$ and validate SR-Rule and ST-Rule
\end{enumerate}

Note that we assume these procedures are executed at the time of $t_j$'s commit, and $t_j$ satisfies RC-Rule. 

\subsection{Validating SR-Rule}

When we generate a version order $\ll^{NWR}$ as described above, $\ll^{NWR}$ always satisfies the rules of NWR except for SR-Rule.
Next, we show how to validate SR-Rule.
Let $S, \ll, t_j$ be a triple of a schedule, a version order for the schedule, and a running transaction that satisfies the rules of NWR except for SR-Rule.

To validate SR-Rule, we must check whether some $t_k$ in $successors_j \cup overwriters_j$ has some path into $t_j$ or not.
We separate the validation into two sub-problem.
At first we show how to validate all $t_k$ in $overwriters_J$.
Next, we show for $successors_j$.

\subsubsection{Validating Overwriters}
\label{sec:tracking_overwriters}

In fact, we already have the implementation; the baseline CC algorithm gives us the necessary component.
The definition of $overwriters_j$ indicates a set of $t_k$ such that $t_j \VORW{} t_k$.
It means that a version $x_i \in rs_j$ is an old version, and there exists a newer version $x_k$.
This definition is completely same with \textit{anti-dependency (r-w dependency)} in CSR \cite{Papadimitriou1986TheControl,Hadzilacos1988ASystems} and in Adya's serialization graph \cite{2000:GIL:846219.847380}.
In other words, $t_j$ is anti-dependent (r-w dependent) on $t_k$ if a transaction $t_k$ is in $overwriters_j$.
Fortunately, because the baseline CC algorithm ensures serializability, we always have the implementation of anti-dependency validation.
For example, S2PL \cite{Gray1992TransactionTechniques} guarantees that $overwriters_j = \phi$.
Silo \cite{Tu2013SpeedyDatabases} assumes that $overwriters_j = \phi$ (and aborts $t_j$ if this assumption does not hold).
% only if はない．VOが違うかもしれんし
Therefore, we can reuse the implementation of the baseline CC algorithm for collecting and validating $overwriters_j$.

\subsubsection{Validating Successors}
\label{sec:tracking_successors}

For $successors_j$, the implementation is not simple.
Consider a version order for $S$ which does not include any $x_k$ such that $x_j <_v x_k$ for all $x_j \in ws_j$.
In this case, $successors_j$ is always empty.
In other words, if every $x_j$ for all $x_j \in ws_j$ is the latest version, we do not have to consider SR-Rule validation.
In fact, almost all in-memory CC algorithms choose the latest versions by locking and they do not consider SR-Rule.
Thus, there is no generic and reusable implementations like $overwriters_j$.


\begin{algorithm}[h]
  \begin{algorithmic}
    \Require{$t_j, \ll^{NWR}$}
    \State{$T = \{RN(t_k)| t_k \in successors_j\}$}
    \Comment{(1)} % $collect
    \State %CRLF

    \ForAll{$t_m$ in $T$}
    % w-r
    \ForAll{$y_m$ in $ws_m$}
    \ForAll{$y_n$ in $rs_j$}
    \If{$y_m <_v y_n$ or $y_m = y_n$}
    \Comment{(2) $\WR{}$ to $t_j$} % $t_j \to ..., \WR{} t_j$
    \State %CRLF
    \Return{MVSG is not acyclic}
    \EndIf
    \EndFor
    \EndFor

    \State %CRLF
    % rw
    \ForAll{$y_g$ in $rs_m$}
    \ForAll{$y_j$ in $ws_j$}
    \If{$y_g <_v y_j$}
    \Comment{(3) $\VORW{}$ to $t_j$} % $t_j \to ..., \VORW{} t_j$
    \State %CRLF
    \Return{MVSG is not acyclic}
    \EndIf
    \EndFor
    \EndFor
    \EndFor
    \State{} % CRLF

    \Return{MVSG is acyclic}
  \end{algorithmic}
  \caption{validation of $successors_j$, where $<_v \in \ll^{NWR}$}
  \label{alg:successors_validation_pseudo}
\end{algorithm}

Figure \ref{alg:successors_validation_pseudo} summarizes how our NWR-extended protocols find cyclic paths.
The key point of our method is to focus and find the last edge of cyclic paths.
We validate whether or not the last edge $\to t_j$ exists, for each three type of edges.
In (1), we collect every transaction $t_m$ which is reachable from $t_k \in successors_j$.
Next, (2) and (3) are validations of the acyclicity of MVSG.
Briefly, (2) checks $t_m \to ..., \WR{} t_j$ and (3) checks $t_m \to ..., \VORW{} t_j$.
(2) validates that some $y_n$ in $rs_j$ is newer than $y_m$ in $ws_m$ for some $t_m$.
If it holds, there is a path to $t_j$ from $t_k$ including $\WR{}$ edge, and MVSG is not acyclic.
Likewise, (3) validates that some $y_j$ in $ws_j$ is newer than $y_g$ in $rs_m$ for some $t_m$.
If it holds, there is a path $t_j$ from $t_k$ including $\VORW{}$ edge, and MVSG is not acyclic.
Note that RC-Rule ensures that any transaction $t_m$ does not have a path $t_m \VOWW{} t_j$ because the edge $\VOWW{}$ is added into MVSG only if some transactions read some $x_j \in ws_j$.
Therefore, if we pass validations (2) and (3), and RC-Rule is satisfied, any edge from any $t_k \in successors_j$ cannot reach into $t_j$.

A key observation is that we assume that we have both read-sets and write-sets for all $t_k \in \{successors_j\}$ and for all $t_i \in RN(t_k)$.
This assumption causes huge overhead since it means that transactions must store their read-set and write-set into shared memory.
In the next section, we show that how to store and maintain both read-set and write-set with tiny overhead.


==> IWR-paper copy/tex/conclusion.tex <==
\section{Conclusion}
In this paper we have formalized the notion of omitting allowed by T/O with TWR, and we have presented the Non-visible write rule (NWR) for any concurrency control protocols.
With NWR, any protocol can in theory be extensible to NWR-extended protocols, which validates the additional version order to omit write operations with preserving both strict serializability and recoverability.
Especially in the workloads that contain blind-updates, our approach of validating the additional version order improves the performance efficiently.
We implemented three NWR-extended protocols, Silo+NWR, TicToc+NWR, and MVTO+NWR, to evaluate the performance gain of our approach.
Experimental results demonstrate that Silo+NWR outperforms the original Silo by more than 11x in the highly contended YCSB-A; meanwhile, every NWR-extended protocol has comparable performance with the original, even in the worst-case on TPC-C.


==> IWR-paper copy/tex/design_overview.tex <==
\section{NWR-extended protocols}
\label{sec:design_overview}

To fully utilize the notion of omittability, we have to consider a new approach to generate version orders, not depending on any implementation of existing protocols.
In this section, we propose a novel technique to extend existing protocols by \textit{validating the additional version order $\ll^{NWR}$}.
We extend existing protocols to generate the additional version order $\ll^{NWR}$ and validate its correctness with an additional algorithm.
We call the protocols that have extended based on our technique as \textbf{``NWR-extended protocols''}.
Our approach is based on the principle that any protocol can in theory generate and validate any number of version orders.
In Section \ref{sec:control_flow}, we show the overview of NWR-extended protocols and clarify how to generate the additional version order $\ll^{NWR}$.
In Section \ref{sec:invisiblewriterule}, we define NWR, a formal condition for a version order to preserve the correctness.
In Section \ref{sec:validation_overview}, we show the validation of the $\ll^{NWR}$'s correctness, derived from NWR.

\subsection{Control Flow}
\label{sec:control_flow}

We now explain the overview of how to extend existing protocols.
Figure \ref{fig:flowchart} depicts the control flow of NWR-extended protocols.
We assume a \textit{baseline protocol}, which preserves strict serializability and recoverability, and assume a running transaction $t_j$ is requesting to commit.
Of course when we do not omit any operations in $t_j$, the baseline protocol ensures the correctness; however, NWR-extended protocols interrupt the baseline protocol at $t_j$'s commit request and try to omit all write operations in $t_j$.
We assume that the selected $t_j$ already satisfies recoverability, and a given version order $\ll$ makes MVSG acyclic in the current schedule $S$ such that $c_j$ and $a_j$ are not in $S$.

\textbf{Generate the additional version order.}
At first, NWR-extended protocols generate an additional version order $\ll^{NWR}$.
It should be done at a reasonable cost, but unfortunately, the computational cost of finding all possible version orders is NP-Complete \cite{Bernstein1983MultiversionAlgorithms,Papadimitriou1982OnVersions}.
% TODO 全探索ではなくてきとうにひとつ選んで作ってみるという選択をしていることを書けてない
To reduce the computational cost, we add a component of \textbf{the pivot version}, denoted as $x_{pv}$, for each data item in order to generate an additional version order $\ll^{NWR}$ and validate it.
The pivot versions are the landmark for generating $\ll^{NWR}$;
NWR-extended protocols generate $\ll^{NWR}$ such that $x_j$ is the version just before $x_{pv}$ for all $x_j$ in $ws_j$ and differences between $\ll$ and $\ll^{NWR}$ are always within data items $x_j$ in $ws_j$.
It means that the two graphs $MVSG(S, \ll)$ and $MVSG(S, \ll^{NWR})$ are isomorphic.
%So $\ll^{NWR}$ does not violate the correctness until $c_j$ is added into $S$.
It is unnecessary to generate and validate the whole MVSG for $\ll^{NWR}$; only a connected subgraph, which includes $t_j$, is necessary for validations.

\textbf{Validations of the correctness.}
We next add two components for validation of the correctness.
These components validate that the pair of $S \cup \{c_j\}$ and $\ll^{NWR}$ does not violate serializability and strict serializability.
For serializability, we check the acyclicity of $MVSG(S \cup \{c_j\}, \ll^{NWR})$.
For strict serializability, we check $t_j$ and all $t_{pv}$, that wrote $x_{pv}$, are concurrent.
Note that strict serializability allows reading or writing old versions only among concurrent transactions, and subsequent non-concurrent transactions must read the latest versions for all data items.
Hence, all $x_j$ in $ws_j$ must be non-latest versions to omit them with the guarantee of non-visibility.
The version order $\ll^{NWR}$ based on the pivot versions always satisfies this condition.

\begin{figure}[t]
    \includegraphics[width=0.45\textwidth]{img/flowchart.pdf}
   \caption{The control flow of NWR-extended protocols.} 
    \label{fig:flowchart}
\end{figure}


\textbf{CAS to ensure atomicity.}
After validations, NWR-extended protocols execute compare and swap (CAS) \cite{Guide2011IntelManual,Technology2012AMD64Date} operations to ensure atomicity of validations.
When all validations and CAS operations pass, then the generated schedule with $\ll^{NWR}$ preserves the correctness; and thus, NWR-extended protocols go to omit all write operations of $t_j$ and commit $t_j$ without any exclusive locking, buffer update, index update, and logging.
In Section \ref{sec:mergedsets_update} we describe the more details of lock-free updates.

\textbf{No false aborts.}
For the case of validation failures, NWR-extended protocols transfer the control to baseline protocols.
Then baseline protocols validate serializability and strict serializability again with their version order, and they determine $t_j$'s termination operation.
Notably, all added components in the control flow do not abort $t_j$ directly.
Only baseline protocols can abort $t_j$.
Our technique offers some overhead for added components but does not increase the abort ratio of transactions.

\textbf{Updating the pivot versions.}
The validations of strict serializability tell us an important observation of how to update the pivot versions.
If we choose a not suitable version as a pivot version $x_{pv}$, validations always fail.
From the definition of MVSG, if $x_{pv}$ is generated by a ``read-modify-write'' operations, the validation of serializability always fails.
More precisely for a running transaction $t_j$, if there exists read-modify-write $r_k(x_i)w_k(x_k)$ and $\ll^{NWR}$ includes $x_i <_v x_j <_v x_k$, MVSG always has the cyclic path $t_k \VORW t_j \VOWW{} t_k$.
Therefore, for serializability, the pivot versions should be updated by \textit{blind-writes} \cite{Weikum2001TransactionalRecovery}.
Furthermore, strict serializability indicates another restriction.
If $\ll^{NWR}$ includes $x_j <_v x_{pv}$ and $t_{pv}$ is not concurrent with $t_j$, strict serializability is violated and the validation fails.
Now we obtain the next proposition:
\begin{proposition}
  A write operation is omittable with the correctness only if there exists another concurrent \textit{blind-write} operation.
\end{proposition}
From this we update the pivot versions in the case a running transaction $t_j$ execute $x_j$ such that $w_j(x_j)$ is blind-write.
This observation also tells us that inserting operations can update the pivot versions, but they are not omittable with the correctness.
For an inserting operation $w_j(x_j)$, the other blind-write is only $w_0(x_0)$.
Clearly $t_0$ is not concurrent with $t_j$ and thus the control flow fails to omit $w_j(x_j)$.

\subsection{Non-visible Write Rule}
\label{sec:invisiblewriterule}

We next define \textbf{Non-visible Write Rule (NWR)}, the formal condition for the additional version order, to clarify what kind of version order preserves the correctness and how to validate strict serializability in the control flow.
NWR consists of five rules: non-visible property rule (NV-Rule), preserving version order rule (PV-Rule), recoverability rule (RC-Rule), serializability rule (SR-Rule), and strict serializability rule (ST-Rule).
NV-Rule forces that all $t_j$'s write operations are non-latest versions, and they are omittable.
PV-Rule forces that the difference between $\ll$ and $\ll^{NWR}$ must be only related to data items $x_j$ in $ws_j$.
As has been noticed above, this rule efficiently reduces the computational cost.
Remaining the three rules are derived straightforwardly from the definition of serializability \cite{Bernstein1983MultiversionAlgorithms}, strict serializability \cite{Herlihy1990Linearizability:Objects}, and recoverability \cite{Hadzilacos1988ASystems}, respectively.

\begin{definition}[Non-visible Write Rule]
  \label{def:invisiblewriterule}
  Let $S, \ll, t_j$ be a schedule, a version order for $S$, and a running transaction such that $t_j \in trans(S) \land c_j, a_j \notin S$, respectively.
  Let $S$ be recoverable, $MVSG(S, \ll)$ be acyclic, and $S$ be strictly serializable.
  % NOTE if there existsにするか for a version orderにするか問題というのがある．
  % 論点はST-Ruleの２つ目のconditionと密接に関係している．
  % すべてのプロトコルについて汎用的な条件とするか，より絞ってomittable を含むversion orderについての条件とするか．
  % ↓定義なのに命題になってるweikumパターンの書き方
  % A version order $\ll'$ satisfies NWR if the following rules are satisfied:
  For a version order $\ll'$, we define NWR as follows:

  \begin{description}
    \item [ \ \ NV-Rule] \mbox{}\\
           $\forall x_j \exists x_k (x_j \in ws_j \Rightarrow  x_j <_v' x_k)$ where $<_v'$ in $\ll'$

    \item[  \ \ PV-Rule] \mbox{}\\
          $\forall x_i \forall x_k ((x_i,x_k \in \{x\} \land x_i \ne x_k \ne x_j \land x_i <_v x_k) \Rightarrow x_i <_v' x_k)$ where $<_v$ in $\ll$ and $<_v'$ in $\ll'$

    \item[  \ \ SR-Rule] \mbox{}\\
          %$\forall t_k (t_k \in RN(t_j) \Rightarrow t_j \notin RN(t_k))$
          $t_j \notin RN(t_j)$

    \item[  \ \ ST-Rule]\mbox{}\\
          $\forall t_k \exists p_j ((t_k \in RN(t_j) \land p_j \in t_j) \Rightarrow  p_j <_S c_k)$ where $<_S$ in $S$

    \item[  \ \ RC-Rule] \mbox{}\\
          $\forall x_i(x_i \in rs_j \Rightarrow c_i \in S)$

  \end{description}
  where $RN$ is defined on $MVSG(S \cup \{c_j\}, \ll')$.
\end{definition}

The following theorem states that if NWR is satisfied, a protocol can commit $t_j$ with the correctness:

\begin{theorem}[Correctness]
  \label{theo:NWR_is_correct}
  If a version order $\ll'$ satisfies NWR,
  $S \cup \{c_j\}$ is strictly serializable and recoverable.
\end{theorem}

The proof is given in Appendix \ref{sec:proof}.

Hence, if a version order $\ll^{NWR}$ generated by NWR-extended protocols satisfies NWR, a running transaction $t_j$ can in theory omit all write operations with the correctness.


\subsection{Validation Overview}
\label{sec:validation_overview}
At the time a running transaction $t_j$ is selected and $\ll^{NWR}$ is generated based on the pivot versions, it is clear that the rules of NWR are satisfied except SR-Rule and ST-Rule.
We next explain the overview of validations for these two rules.
A key observation is that both rules collect and validate reachable transactions $RN(t_j)$.
We now separates directly reachable transactions into two sets:
  $$overwriters_j := \{t_k| t_j \VORW{} t_k \in MVSG(S, \ll^{NWR})\}$$
  $$successors_j := \{t_k| t_j \VOWW{} t_k \in MVSG(S, \ll^{NWR})\}$$
The following theorem is then immediate:

\begin{theorem}[Reachable transactions]
  \label{theo:what_are_RN}
  If RC-Rule is satisfied, then any path in $RN(t_j)$ is starting from $t_j \to t_k$ such that $t_k$ is in $overwriters_j$ or $successors_j$.
\end{theorem}
\begin{proof} (sketch)
As we have been noted in Section \ref{sec:def_of_mvsg}, edges of MVSG are distinguished the three types: $\WR{}, \VORW{}$, and $\VOWW{}$. 
Since RC-Rule is satisfied and $S$ is recoverable, there does not exist any edge $\WR{}$ starting from $t_j$; no committed transactions read any version $x_j$ in $ws_j$.
Therefore, the type of an edge $t_j \to t_k$ for any $t_k$ is always either $\VORW{}$ or $\VOWW{}$.
\end{proof}

So we can separate the validation of NWR-extended protocols into two sub-validations related to $successors_j$ and $overwriters_j$.
We now summarize the additional validations of NWR-extended protocols as follows: for each $t_k$ in $overwriters_j$ or $successors_j$, (1) checking $t_k$ is not reachable into $t_j$ (SR-Rule), and (2) checking $t_k$ is concurrent with $t_j$ (ST-Rule).

\subsubsection{Validation of overwriters}
We next show that it is not necessary to invent validations for $overwriters_j$.
Since elements of $overwriters_j$ depends on $t_j$'s read operations, and our approach focuses only on write operations, transactions of $overwriters_j$ are never changed from baseline protocols.
Therefore, there exist reusable validation algorithms.
We next show how to validate $overwriters_j$ for each SR-Rule and ST-Rule.

\textbf{SR-Rule validation of overwriters.}
If some transaction $t_k$ in $overwriters_j$ violates SR-Rule, there exists some path $t_j \VORW{} t_k \to  ... \to t_j$.
That is, some version $x_i$ in $rs_j$ is overwritten by $t_k$.
This type of edge is well-known as the \textit{anti-dependency} \cite{2000:GIL:846219.847380, Papadimitriou1986TheControl, Hadzilacos1988ASystems} and all serializable protocols can detect or prevent the cycles starting from an anti-dependency edge by using lockings \cite{Gray1992TransactionTechniques}, timestamps \cite{Reed1978NamingSystem.}, or validation phases \cite{Kung1981OnControl}. 
Thus, we can reuse implementations of baseline protocols straightforwardly.

\textbf{ST-Rule validation of overwriters.}
If some transaction $t_k$ in $overwriters_j$ violates ST-Rule, there exists some too old version $x_i$ in $rs_j$; however,  $t_j$ cannot read such stale versions since baseline protocols ensure strict serializability.
Thus, we do not have to consider ST-Rule validation of $overwriters_j$.

\subsubsection{Validation of successors}
\label{sec:validation_overview}
We have seen that it is unnecessary to validate $overwriters_j$; however, we have to add new validations for $successors_j$.
Algorithm \ref{alg:successors_validation_pseudo} provides the pseudo-code of the validations of both SR-Rule and ST-Rule for $successors_j$.
In (A) of Algorithm \ref{alg:successors_validation_pseudo}, we collect every transaction $t_m$ such that $t_m$ is in $successors_j$ or $t_m$ is reachable from $t_k$ in $successors_j$.
In (B), we validate ST-Rule by checking the concurrency of all $t_m$ and $t_j$.
Next, (C) and (D) are validations of SR-Rule.
We focus and find the last edge $t_m \to t_j$ in cyclic paths.
%If there exists a cyclic path starting from some $t_k$, the last edge $\to t_j$ for every three types of edges.
Note that any transaction $t_m$ does not have a path $t_m \VOWW{} t_j$ since $S$ is recoverable; the edge $\VOWW{}$ is added into MVSG only if some committed transactions read some $x_j$ in $ws_j$ (it is impossible because of RC-Rule).
Therefore, we need only to check the two types of the last edge $t_m \WR{} t_j$ and $t_m \VORW{} t_j$; (C) checks the former and (D) checks the latter.
(C) validates that some $y_n$ in $rs_j$ is newer than $y_m$ in $ws_m$ for some $t_m$.
If it holds, there exists a cyclic path $t_j \VOWW{} ... \to t_m \WR{} t_j$.
Likewise, (D) validates that some $y_j$ in $ws_j$ is newer than $y_g$ in $rs_m$ for some $t_m$.
If it holds, there exists a cyclic path $t_j \VOWW{} ... \to t_m \VORW{} t_j$.
Consequently, when we pass validations (C) and (D), any $t_k$ in $successors_j$ is not reachable into $t_j$.


\begin{algorithm}[t]
  \begin{algorithmic}
    \Require{$t_j, \ll^{NWR}$}
    \State{$T = \{t_k, t_i | t_k \in successors_j \land t_i \in RN(t_k) \}$}
    \Comment{(A)} % $collect
    \State %CRLF

    \ForAll{$t_m$ in $T$}

    \If{$t_m$ commits before $t_j$'s beginning}
      \Comment{(B)} % ST-Rule
      \State %CRLF
      \Return{ST-Rule is not satisfied}
    \EndIf
    
    \State %CRLF


    % w-r
    \ForAll{$y_m$ in $ws_m$}
    \ForAll{$y_n$ in $rs_j$}
    \If{$y_m <_v y_n$ or $m = n$}
    \Comment{(C) $\WR{}$ to $t_j$} % $t_j \to ..., \WR{} t_j$
    \State %CRLF
    \Return{MVSG is not acyclic}
    \EndIf
    \EndFor
    \EndFor

    \State %CRLF
    % rw
    \ForAll{$y_g$ in $rs_m$}
    \ForAll{$y_j$ in $ws_j$}
    \If{$y_g <_v y_j$}
    \Comment{(D) $\VORW{}$ to $t_j$} % $t_j \to ..., \VORW{} t_j$
    \State %CRLF
    \Return{MVSG is not acyclic}
    \EndIf
    \EndFor
    \EndFor
    \EndFor
    \State{} % CRLF

    \Return{MVSG is acyclic}
  \end{algorithmic}
  \caption{validations for $successors_j$ where $<_v$ in $\ll^{NWR}$}
  \label{alg:successors_validation_pseudo}
\end{algorithm}


==> IWR-paper copy/tex/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
We now show our evaluation of three NWR-extended protocols: Silo+NWR \cite{Tu2013SpeedyDatabases}, TicToc+NWR \cite{Yu2016Tictoc:Control}, and MVTO+NWR \cite{Reed1978NamingSystem.,Bernstein1982ConcurrencySystems, Lim2017Cicada:Transactions}.
Our focus of the evaluation is to clarify the followings:

\begin{itemize}
  \setlength\itemsep{0.15em}
\item{Effectiveness: omittable write operations improve the performance in write-contended workloads.}
\item{Low-overhead property: Every NWR-extended protocol keeps comparable performance to the original, even in read-intensive workloads.}
\item{Limitation: our approach is efficient only in the case when the workload contains blind-writes.}
\end{itemize}

The performance results demonstrate that, if workloads contain blind-writes, our approach is useful for both read-intensive and write-intensive workloads.

\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{img/whatisfv.pdf}
  \caption{Overall structure of our prototype}
  \label{fig:whatisfv}
\end{figure}

\subsection{Experimental Setup}

For experiments, we implement our prototype: a lightweight, non-distributed, and embedded transactional key-value storage written in C++.
Our prototype consists of in-memory storage, various CC algorithms, a tree-based index forked by Masstree \cite{Mao2012CacheStorage}, and a parallel-logging manager \cite{Zheng2014FastParallelism, Johnson2010Aether:Logging}.
Figure \ref{fig:whatisfv} shows the overall structure of our prototype.
Every leaf-node of the index has the pointer to an indirection.
Each indirection includes a) 64-bits pointer to the data item and b) the pivot version object described in Section \ref{sec:implementation}.
Each data item is represented as a linked-list ordered by versions as newest-to-oldest.
For all single-version protocols, every linked-list always consists of a single node.

We deploy all experiments on a 144-core machine with four Intel Xeon E7-8870 CPUs and 1TB of DRAM.
Each CPU socket has 18 physical cores and 36 logical cores by hyperthreading.
The results of experiments in over 72 cores may show sub-linear scaling due to contention within physical cores.
Each socket has 45MB L3 shared cache.
Each worker thread allocates the memory from separated space specified with the Linux numactl.
We compile all queries at build time, and thus our experiments do not use both networked clients and SQL interpreters.
Each worker thread has the thread-local workload generator to input transactions by itself.

\subsubsection{Extension details}
In our experiments, we extend the following three state-of-the-art protocols:

\textbf{Silo.}
This optimistic protocol adopts the backward validation \cite{Kung1981OnControl}, and the epoch-based group commit.
Silo generates a version order by exclusive lockings.
When a transaction $t_j$ requests to commit, Silo acquires exclusive lockings for all $x_j$ in $ws_j$.
Locking ensures that all $x_j$ are the latest versions, and thus $successors_j$ is always empty set.
The validation of $overwriters_j$ in Silo checks $overwriters_j = \phi$.
If a data item $x_i$ in $rs_j$ is overwritten and there exists a newer version, Silo aborts $t_j$.
To extend Silo to Silo+NWR, we expand the 64-bits per data item transaction-id objects into the 128-bits pivot version objects.
In Silo, each transaction id object stores 1) 32-bits epoch, 2) 31-bits per-epoch version number, and 3) 1-bit exclusive lock flag.
We expand these objects into 128-bits and add mRS and mWS into the rest 64-bits.

\textbf{TicToc.}
This optimistic protocol adopts a more sophisticated validation algorithm for $overwriters_j$ than Silo.
TicToc adds read-timestamps into Silo's transaction id objects.
Even if a version $x_i$ in $rs_j$ is overwritten (it means $overwriters_j \ne \phi$), TicToc validates read-timestamps to commit $t_j$.
TicToc generates the same version order as Silo; TicToc acquires exclusive lockings for all $x_j$ in $ws_j$, and thus each version $x_j$ is the latest version of $x$.
To extend TicToc to TicToc+NWR, we compress the original encoding of the 64-bits transaction-id objects into 32-bits and store the epoch number into the rest 32-bits.

\textbf{MVTO.}
We implemented MVTO based on Cicada \cite{Lim2017Cicada:Transactions};
we apply the per-thread distributed timestamp generation (multi-clock), read sets for optimistic multi-versioning, and rapid garbage collection.
Unfortunately, Cicada's multi-clock does not ensure strict serializability.
It ensures only causal consistency \cite{Lim2017Cicada:Transactions}.
To ensure strict serializability, we apply the epoch-based group commit to both MVTO and MVTO+NWR, by expanding the 64-bits timestamp objects into the 128-bits pivot version objects with epoch numbers.
Note that MVTO aborts a transaction if its write set is invalid, in contrast with the fact that Silo and TicToc validate their read set.
Since the protocol of MVTO ensures that all transactions in $overwriters_j$ cannot be reachable into the running transaction $t_j$, MVTO executes only the validation for $successors_j$.
Hence, we do not have the reusable implementation of validation for $overwriters_j$ within MVTO.
To validate $overwriters_j$, we use the Silo's tiny implementation.
When a version $x_i$ in $rs_j$ is not the latest version of the data item, then MVTO+NWR determines that MVSG might be cyclic and cannot commit $t_j$ with $\ll^{NWR}$.


\subsubsection{Benchmarks}
We select two benchmarks for performance evaluation: YCSB \cite{Cooper2010BenchmarkingYCSB} and TPC-C \cite{10.5555/1946050.1946051}.

\textbf{YCSB.}
This workload generator is representative of current large-scale on-line benchmarks.
YCSB provides various workloads, and we choose YCSB-A (write-intensive) and YCSB-B (read-mostly) for benchmarking.
Since the original YCSB does not support a transaction with multiple operations,
we implemented a YCSB-like workload generator within our prototype.
In our implementation, each transaction accesses four data items chosen randomly based on Zipfian distribution with a parameter $\theta$.
Each data item has a single primary key and an 8-bytes additional column.
We populate our prototype as a single table with 100K data items.
That is, our prototype is always fitted in memory for all single-version protocols.
In this workload, we show how efficient NWR is for contended workloads.

\textbf{TPC-C.}
This workload is the classical industry-standard benchmark for evaluating the performance of transaction processing.
It consists of six tables and five transactions that simulate an information system of a wholesale store.
TPC-C is the write-intensive and low contention workload.
A key point of the TPC-C benchmark is that there exist only blind-inserts.
All other write operations in TPC-C are read-modify-write; they must read the latest versions to write the next versions and always fail to validate SR-Rule.
Therefore, we cannot omit any write operations in TPC-C.
In this workload, we focus on how much performance drops by our extension.

\subsection{YCSB Benchmark Results}
\label{sec:ycsb}

\subsubsection{YCSB-A: read-write mixed workload}
YCSB-A defines the proportion of operations as 50\% read and 50\% blind-write.
A key observation of this workload is that a substantial proportion of write operations are omittable.
In YCSB, all data items must be initialized before experiments \cite{Cooper2010BenchmarkingYCSB}; thus, all write operations are blind-writes.
That is, the validation failure of $\ll^{NWR}$ is rarely happen in NWR-extended protocols.
Once the latest versions for each 40ms epoch are updated, other write operations do not violate ST-Rule.
Besides, for SR-Rule, it is rare to fail the validation of $successors_j$.
This is because blind-writes reduce the number of edges in MVSG with $\ll^{NWR}$; since a transaction $t_j$ trying to omit $w_j(x_j)$ does not have read any $x_k$ in $\{x\}$, there is no cyclic path $t_j \VOWW{} t_{pv} \WR{} t_j$ for data item $x$.  
Thus, NWR-extended protocols are expected to generate a tremendous number of omittable write operations and improve performance.


\textbf{Efficiency of NWR-extended protocols.}
Figure \ref{fig:ycsb-a-high} shows the results on the YCSB-A workload with high contention rate ($\theta = 0.9$).
Prior work shows that recent protocols suffer from this write contended workloads \cite{Wu2017AnControl, Yu2014StaringCores, Kim2016Ermia:Workloads, Fan:2019:OVG:3342263.3360357}.
We later show the performance results in the same workload with variable contention rates.
With up to 21 threads, the throughput of all protocols increases as the number of threads increases.
Beyond 41 threads, coordination such as exclusive locking hurts the performances of baseline protocols.
This is because our environment has only 36 cores per single CPU socket.
Cache-coherence traffic occurred by exclusive locking degrades their throughput significantly.
However, the performances of NWR-extended protocols in YCSB-A are not limited.
When the number of thread increased, NWR-extended protocols outperform originals.
In the best case at 144 threads, the throughput of NWR-extended algorithms is more than 11x better than originals.


\begin{figure}[t]
  \centerline{
    \subfloat{
      \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend.pdf}
    }
  }
  \vspace{-10pt}
  \addtocounter{subfigure}{-1}
  \centerline{
    \subfloat{
      \includegraphics[width=0.40\textwidth]{benchmark_figures/ICDE/build/YCSB-a-Contention9-TableSize100000_tps-a-tps.pdf}
    }
  }
  \vspace{-6pt}
  \caption{YCSB-A Benchmark results with $\theta=0.9$}
  \label{fig:ycsb-a-high}
\end{figure}

\begin{table}[t]
  \begin{tabular}{|l|c|c|}
    \hline
    Protocols & Commit ratio & Commit ratio with \tiny{$\ll^{NWR}$} \\
    \hline \hline
    Silo+NWR & 94 & 85 \\
    TicToc+NWR & 98 & 65 \\
    MVTO+NWR & 98 & 72  \\
    \hline
  \end{tabular}
  \caption{Commit ratio (\%) of the additional version order $\ll^{NWR}$, generated by NWR-extended protocols, on YCSB-A at 144 threads.}
  \label{tab:commit_ratio}
\end{table}


\begin{figure*}[t]
  \vspace{-10pt}
    \subfloat[
    At 1 thread
    ]{
      \includegraphics[width=0.42\textwidth]{benchmark_figures/ICDE/build/YCSB-a-FixedThread1-FixedTableSize100000-Contention9_breakdown-aggregated.pdf}
      \label{fig:ycsb-breakdown-a-1}
    }
    \hspace{-10pt}
    \subfloat[
     At 144 threads
     ]{
      \includegraphics[width=0.42\textwidth]{benchmark_figures/ICDE/build/YCSB-a-FixedThread144-FixedTableSize100000-Contention9_breakdown-aggregated.pdf}
      \label{fig:ycsb-breakdown-a-144}
    }
    \hspace{-24pt}
    \subfloat{
      \includegraphics[width=0.17\textwidth]{benchmark_figures/ICDE/legend_breakdown.pdf}
      \label{fig:ycsb-breakdown-a-144}
    }
  
  \caption{Runtime breakdowns of Figure \ref{fig:ycsb-a-high}}
  \label{fig:ycsb-breakdown}
  \end{figure*}


\begin{figure}[t]
  \centerline{
    \subfloat{
      \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend.pdf}
    }
  }
  \vspace{-10pt}
  \addtocounter{subfigure}{-1}
  \centerline{
    \subfloat{
      \includegraphics[width=0.40\textwidth]{benchmark_figures/ICDE/build/YCSB-a-VariableContention-FixedThread144-TableSize100000-a-tps.pdf}
    }
  }
  \vspace{-6pt}
  \caption{YCSB-A Benchmark results with variable $\theta$}
  \label{fig:ycsb-variable-contention}
\end{figure}

\textbf{Differences between baseline protocols.}
The results for YCSB-A also shows that TicToc+NWR and MVTO+NWR do not scale, unlike Silo+NWR.
The main reason for the performance gap is that TicToc and MVTO allow \textit{reading old versions}.
When a transaction reads a non-latest version that has already overwritten, Silo must abort the transaction, but TicToc and MVTO do not.
They may commit the transaction if their validation pass, and thus mRS in the pivot version storage may be updated with lower version numbers at any time.
Recall that the validation (4) in Algorithm \ref{alg:successors_validation} fails when a version number $y_g$ in mRS is lower.
Therefore, reading old versions decreases the commit ratio of NWR-extended protocols with $\ll^{NWR}$.
Table \ref{tab:commit_ratio} lists the commit ratio of the additional version order $\ll^{NWR}$ for each NWR-extended protocols.
Although the commit ratio of TicToc+NWR and MVTO+NWR are better than Silo+NWR, they sometimes give up to omit write operations in the validation of $\ll^{NWR}$.
In contrast, Silo+NWR efficiently commits transactions with $\ll^{NWR}$ and omits write operations.
It is known that the validation algorithm of Silo has higher false abort rates \cite{Yu2016Tictoc:Control, Yuan2016BCC:Databases, Ding2018ImprovingOptimistic}; however, it is favorable for our approach with $\ll^{NWR}$.


\textbf{Runtime breakdown.}
Figure \ref{fig:ycsb-breakdown-a-1} and \ref{fig:ycsb-breakdown-a-144} show the runtime breakdown of committed transactions at a single and 144 threads on the YCSB-A with $\theta = 0.9$, respectively.
``NWR\_OVERHEAD'' indicates the additional components of our approach described in Section \ref{sec:control_flow}.
At a single thread, the top consumer of CPU ticks is INDEX for all protocols, but the overhead of NWR is not negligible for all NWR-extended protocols.
Compared to Silo+NWR, TicToc+NWR and MVTO+NWR spend more CPU ticks for the additional components since they adopt the different approaches for validation of $overwriters_j$.
Recall that TicToc and MVTO allow reading old versions, but Silo does not; thus, they spend more ticks on updating mRS for each pivot version.
At 144 threads, the primary consumers of CPU-ticks shift to LOCKWAIT, and the overhead of NWR becomes negligibly small.
NWR-extended protocols dramatically reduce the CPU ticks wasting for locking by generating omittable write operations.
Note that MVTO, which shows the lowest performance in Figure \ref{fig:ycsb-a-high}, spent fewer CPU ticks per single transaction than Silo and TicToc.
This is because our runtime breakdown measures only the CPU ticks on concurrency control protocols for committed transactions.
Other overheads such as malloc for creating new versions or lock-wait for aborted transactions are not shown in this figure, and they are current bottlenecks.
We remain cache-efficient optimization for MVTO and MVTO+NWR as future work.



\begin{figure}[t]
  \centerline{
    \subfloat{
      \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend_only_silo.pdf}
    }
  }
  \vspace{-10pt}
  \addtocounter{subfigure}{-1}
  \centerline{
    \subfloat{
      \includegraphics[width=0.40\textwidth]{benchmark_figures/ICDE/build/YCSB-A-VariableEpoch-a-tps.pdf}
    }
  }
  \vspace{-6pt}
  \caption{YCSB-A Benchmark results with variable epoch durations}
  \label{fig:ycsb-variable-epoch}
\end{figure}

\subsubsection{YCSB-A with variable contention rates.}
Next, we experiment YCSB-A with variable contention rates.
Figure \ref{fig:ycsb-variable-contention} shows the results at 144 threads.
Once the contention rate exceeds 0.7, the throughputs of Silo+NWR and TicToc+NWR drops due to exclusive locking for write operations.
MVTO suffers from cache-coherence traffic caused by multiversion storage.
In MVTO, it is unnecessary to acquire exclusive locking for write operations, but instead, memory allocation for creating new versions is needed, and it limits the throughput.
At the contention rate of 0.99, every baseline protocol presents almost the same throughput.
Previous studies show the same trend with this result \cite{Fan:2019:OVG:3342263.3360357, Yu2014StaringCores, Wu2017AnControl}.
However, NWR-extended protocols outperform the originals and do not degrade the throughput when the contention rate increased.
Furthermore, Silo+NWR improves performance at the contention rate of 0.99.
In this setting, transactions request to read or write to the same data items, and Silo+NWR successes to omit almost all write operations.
Therefore, almost all read operations receive the same versions, which are already stored in the CPU caches.
Compared to Silo+NWR, MVTO+NWR and TicToc+NWR do not degrade but cannot improve performance in this setting, since they allow \textit{reading old versions} as has been noted above.


\subsubsection{YCSB-A with variable epoch durations.}
As has been shown in Section \ref{sec:implementation}, NWR-extended protocols ensure ST-Rule by using epoch-based group commits.
Transactions in the same epoch are concurrent and satisfy ST-Rule for any version order.
Hence, the longer epoch duration will make more transactions concurrent and decrease the validation failure of ST-Rule.
To investigate the effect of epoch duration, we experiment YCSB-A with variable epoch duration.
Figure \ref{fig:ycsb-variable-epoch} depicts the throughputs of Silo and Silo+NWR.
The original Silo shows unstable performance as the epoch duration increases.
This is because the longer epoch duration causes larger commit buffers for each epoch.
In contrast, the throughput of Silo+NWR grows as the epoch duration increases since the ST-Rule validation failures decrease.
Thus, we can improve performance by increasing the epoch duration as long as applications allowed.


\subsubsection{YCSB-B: read-mostly workload}
Figure \ref{fig:ycsb-b-high} shows the performance results on the read-mostly workload.
YCSB-B is expected as not suitable for our approach since it defines the proportion of read operation as 95\%; that is, concurrent write operations into the same data item are rarely observed.
However, NWR-extended protocols show comparable performances with the originals, and surprisingly, Silo+NWR outperforms Silo.
This gain comes from the observation that omitting write operations have a good effect on the other transactions.
In this case, Silo+NWR replaces overwriting operations to omittable write operations, and it prevents the validation failure of other transactions.
Figure \ref{fig:ycsb-b-high-abort} shows the number of aborts in the same experiment.
Here we see Silo+NWR reduces the abort rate of the original Silo, and it provides the performance improvement in this workload.

% 1 column two graph
% \begin{figure}[t]
%   \centerline{
%     \subfloat{
%       \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend.pdf}
%     }
%   }
%   \vspace{-20pt}
%   \addtocounter{subfigure}{-1}
%   \centerline{
%     \subfloat[
%       Throughput
%     ]{
%       \includegraphics[width=0.25\textwidth]{benchmark_figures/ICDE/build/YCSB-b-Contention9-TableSize100000_tps-b-tps.pdf}
%     \label{fig:ycsb-b-high}
%     }
%     \hfill
%     \subfloat[
%       Aborts per second
%     ]{
%       \includegraphics[width=0.25\textwidth]{benchmark_figures/ICDE/build/YCSB-B-Contention9-only-silo-b-aborts.pdf}
%       \label{fig:ycsb-b-high-abort}
%     }
%   }
%   \caption{YCSB-B Benchmark results with $\theta=0.9$}
%   \label{fig:ycsb-tps2}
% \end{figure}

\begin{figure}[t]
  \centerline{
    \subfloat{
      \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend.pdf}
    }
  }
  \vspace{-10pt}
  \addtocounter{subfigure}{-1}
  \centerline{
    \subfloat{
      \includegraphics[width=0.40\textwidth]{benchmark_figures/ICDE/build/YCSB-b-Contention9-TableSize100000_tps-b-tps.pdf}
    }
  }
  \vspace{-6pt}
  \caption{Throughput in YCSB-B with $\theta=0.9$}
  \label{fig:ycsb-b-high}
\end{figure}


\begin{figure}[t]
  \centerline{
    \subfloat{
      \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend_only_silo.pdf}
    }
  }
  \vspace{-10pt}
  \addtocounter{subfigure}{-1}
  \centerline{
    \subfloat{
      \includegraphics[width=0.40\textwidth]{benchmark_figures/ICDE/build/YCSB-B-Contention9-only-silo-b-aborts.pdf}
      }
  }
  \vspace{-6pt}
  \caption{Aborts of Silo and Silo+NWR in YCSB-B}
  \label{fig:ycsb-b-high-abort}
\end{figure}

% ここまで



\subsection{TPC-C Benchmark Results}
\label{sec:tpc-c}

We implement TPC-C in our prototype, the same as the original specifications.
Recall that all five queries in TPC-C do not contain blind-writes without inserting queries.
It means that there are no omittable write operations in this workload.
We consider emerging workloads contains tremendous blind-writes; however, we experiment on this benchmark to illustrate the low-overhead property of our NWR-extended protocols.

\textbf{Overheads of the pivot version storage.}
To better understand the low-overhead property of NWR-extended protocols, we run the TPC-C benchmark with a single warehouse.
This high-contended scenario presents the worst case for NWR since the pivot version storage for each data item will be updated frequently but never be utilized.
Figure \ref{fig:tpcc-tps} shows the achieved throughputs as the number of threads increased.
It can be seen that Silo+NWR and TicToc+NWR's overheads are negligibly small.
The performance degradations in these two NWR-extended protocols are less than 10\%, and they achieved comparable performances with originals.
However, MVTO+NWR presents about 0.84x lower throughput than the original MVTO.
This is because the additional components in MVTO+NWR require traversing version lists twice, and it incurs the performance penalty from cache-coherence traffic. 
%Remind that the pivot version storage is not stored for each version object but stored for each indirection (sentinel node of version lists).
%Thus, MVTO+NWR must retrieve sentinel nodes at the time, updating the pivot version storage.
As we have been noted in Section \ref{sec:implementation}, MVTO+NWR uses Silo's anti-dependency validation; MVTO+NWR validates that there exists some newer version for each $t_k$ in $rs_j$.
This validation requires to traverse the version list again for each $t_k$.
Hence, MVTO+NWR needs to traverse a version list twice per single read operation, once for a read operation, and once for validating $overwriters_j$.
This additional traversing is harmful to the CPU cache, as the number of elements in a version list increases.
In TPC-C, the queries new-order and payment frequently perform read-modify-write into the warehouse and district tables, and the longer version-lists degrades the performance of MVTO+NWR.

% \textbf{Runtime breakdown.}
% Figure \ref{fig:tpcc-breakdown} illustrates the runtime breakdown of the same experiments 144 threads.
% MVTO and MVTO+NWR suffer from traversing multiversion index, but they can read and write multiple versions without exclusive locking.
% Thus, they achieve the highest performances.
% TicToc, Silo, and their extended protocols suffer from waiting for locking in this highly contended scenario since there are no omittable write operations.
% Here, we see the same trend with the YCSB benchmark; the overhead of our approach in NWR-extended protocols is negligibly small at 144 threads.

\begin{figure}[t]
  \centerline{
    \subfloat{
      \includegraphics[width=0.5\textwidth]{benchmark_figures/ICDE/build/legend.pdf}
    }
  }
  \vspace{-10pt}
  \addtocounter{subfigure}{-1}
  \centerline{
    \subfloat{
      \includegraphics[width=0.40\textwidth]{benchmark_figures/ICDE/build/TPCC-Mixed-VariableThread-FixedSingleWarehouse_tps-Mixed-tps.pdf}
    }
  }
  \vspace{-6pt}
  \caption{TPC-C benchmark results with a single warehouse}
  \label{fig:tpcc-tps}
\end{figure}

% \begin{figure}[t]
%       \includegraphics[width=0.45\textwidth]{benchmark_figures/ICDE/build/TPCC-Mixed-FixedThread144-FixedSingleWarehouse_breakdown-aggregated.pdf}
%   \caption{Runtime breakdown of Figure \ref{fig:tpcc-tps} at 144 threads}
%   \vspace{-6pt}
%   \label{fig:tpcc-breakdown}
% \end{figure}


% \begin{figure}[t]
%     \begin{tabular}{cc}
%     \subfloat[
%     At 1 threads]{
%       \includegraphics[width=0.45\textwidth]{benchmark_figures/ICDE/build/TPCC-Mixed-FixedThread1-FixedSingleWarehouse_breakdown-aggregated.pdf}
%     \label{fig:tpcc-breakdown-1}
%     }
%     \\
%     \vspace{-6pt}
%     \subfloat[
%       At 144 threads]{
%       \includegraphics[width=0.45\textwidth]{benchmark_figures/ICDE/build/TPCC-Mixed-FixedThread144-FixedSingleWarehouse_breakdown-committed.pdf}
%     \label{fig:tpcc-breakdown-144}
%     }
%     \end{tabular}
%   \caption{Runtime breakdown for Figure \ref{fig:tpcc-tps}}
%   \label{fig:tpcc-breakdown}
% \end{figure}


==> IWR-paper copy/tex/future_work.tex <==
\section{Future Work}
The following two problems remain as future work:

\begin{enumerate}
\item Can we find the most efficient way to decide the version order based on the all invisible strategy? For a write operation $w_j(x_j)$, a scheduler based on the all invisible strategy can assign $x_j$ anywhere between $x_0$ and the latest version of $x_{latest}$.
Because different version orders generate different MVSGes, the detail of version orders affects the commit rate.

\item How many version orders should be validated? In addition to the version order based on all invisible strategy, we can sometimes improve the commit rate by validating yet another version order. For example, we can consider the strategy for hot (frequently written) data items; a new version of a hot data item is better to be ordered older to omit, and a new version of a cold data item may be better to be ordered the latest. Because LI-Rule is satisfied only when there exists a concurrent write operation, write operations which access cold items are rarely to be IW operations. Thus, "order some write operations to be old, and order others to be the latest" strategy may work well. However, the best strategy and the best amount of validating version orders depend on workload.
\end{enumerate}

If we know a real workload and access patterns of data items, we may be able to extend a conventional scheduler to an NWR scheduler with validating \textit{better} version orders.


==> IWR-paper copy/tex/implementation.tex <==
\section{Lock-free Implementation}
\label{sec:implementation}

We can now validate SR-Rule and ST-Rule with the validation for $successors_j$.
% ↑ほかのcomponentsが明らかでないからいえない
However, the naive implementation of Algorithm \ref{alg:successors_validation_pseudo} has huge overheads since it forces all transactions to store their footprints into shared memory; there is an assumption that we have both $rs_k$ and $ws_k$ for all reachable transactions from $t_k$ in $successors_j$, at the commit request from $t_j$.
To solve this problem, we propose \textbf{the pivot version objects}, which provide the efficient lock-free implementation of NWR-extended protocols.
We embed the pivot version object for each data item $x$.
Each object stores each pivot version $x_{pv}$ and footprints of concurrent transactions that are reachable from $t_{pv}$ on MVSG.
These objects play crucial roles of the control flow of NWR-extended protocols, described in Section \ref{sec:control_flow}.
Briefly, for a transaction $t_j$, we find $x_{pv}$ for all $x_j$ in $ws_j$, generate $\ll^{NWR}$, and validate $successors_j$ by using the pivot version objects.
In Section \ref{sec:the_data_structure}, we explain the layout of the pivot version objects.
In Section \ref{sec:mergedsets_update}, we show the detailed and efficient control flow of NWR-extended protocols in lock-free fashion.

\subsection{Layout of the pivot version objects}
\label{sec:the_data_structure}

Each pivot version object includes four fields: an epoch number, the pivot version (PV), a merged read set (mRS), and a merged write set (mWS).
Figure \ref{fig:datastructure} shows the layout of the pivot version object.

\begin{itemize}

  \item
        \textbf{Epoch.}
        This field holds 32-bits an epoch number, which enables to validate ST-Rule.
        We use \textit{epoch-based group commit} \cite{Tu2013SpeedyDatabases, Chandramouli2018FASTER:Updates} for all NWR-extended protocols.
        Epoch-based group commit divides the wall-clock time into \textit{epochs}, and assigns each transaction into the corresponding epoch.
        Transactions in an epoch are grouped, and their commit operations are delayed until the epoch is \textit{stable}.
        This nature of delaying commit operations is favorable for ST-Rule;
        it enables us to check that two transactions are concurrent in a simple way.
        Since transactions in the same epoch are committed at the same time, we can say that transactions in the same epoch are concurrent.
        The epoch field stores the epoch number of the transaction $t_{pv}$, which write the pivot version of this data item.
        If the epoch number does not match the current ($t_j$'s) epoch, ST-Rule does not satisfied.
        We process the epoch number as the same with Silo \cite{Tu2013SpeedyDatabases}; after all transactions in an epoch are committed, subsequent transactions are assigned in the next epoch.
  \item
        \textbf{The pivot version (PV).}
        This field stores the \textit{version number} of pivot version $x_{pv}$, which enables to generate the additional version order $\ll^{NWR}$.
        Version numbers are decided in the version order $\ll$ given by baseline protocols and reset for each epoch.
        Generally, baseline protocols have per-data item version numbers such as write-timestamp \cite{Yu2016Tictoc:Control,Lim2017Cicada:Transactions} or transaction id \cite{Tu2013SpeedyDatabases}, thus we can reuse them.
        For a running transaction $t_j$, a version number of $x_j$ in $ws_j$ can take two possible values:
        for the additional version order $\ll^{NWR}$, the version number of $x_j$ is given by decrement of $x_{pv}$ since the version $x_j$ is just before version of $x_{pv}$ in $\ll^{NWR}$.
        If $t_j$ does not commit with $\ll^{NWR}$ but commit with a version order $\ll'$ generated by baseline protocols, the version number of $x_j$ must reflect $\ll'$.
        We update this field at the commit of transactions that perform the first \textit{blind-update} for each epoch.
  \item
        \textbf{MergedRS (mRS) and MergedWS (mWS).}
        These fields store mRS and mWS, 32-bits hash table that enable to validate SR-Rule for $successors_j$ described in Section \ref{sec:validation_overview}.
        Figure \ref{fig:merged_sets} illustrates the layouts.
        Each data item $x, y, z, ..., \in D$ is mapped into the corresponding slot by a hash function $h$.
        Each hash table consists of eight 4-bits slots, and stores an union of $rs_k$ or $ws_k$ for all transactions $\{t_k\}$ such that $t_k$ is in $RN(t_{pv})$ or $t_k = t_{pv}$.
        Each $t_k$ stores the version number for each $x_i$ in $rs_k$ and $x_k$ in $ws_k$ into the corresponding slot if the version number is less than the current value, or the current value is zero.
        Each slot holds only the lowest version number as 4-bits integer.
        When a version number is larger than the upper bound of 4-bits integers, we truncate it to $(2^4-1)$.
        These fields reset when the epoch number proceeds.
%, but there exists false positives; two data items might be assigned into the same slot if the hash function generates the same hash value.
\end{itemize}

We encode each field as 32-bits, and thus every data item maintains 128-bits the pivot version object.
On the 64-bits machine with 128-bits atomic operations such as CMPXCHG16B \cite{Guide2011IntelManual,Technology2012AMD64Date}, we can handle the pivot version objects with lock-free fashion.


\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{img/datastructure.pdf}
  \caption{Layout of a pivot version object. It consists of four 32-bits fields.}
  \label{fig:datastructure}
\end{figure}

\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{img/mergedsets.pdf}
  \caption{mRS and mWS are 32-bits hash table consisting of eight 4-bits version numbers. The version number reflects the given version order $\ll$.}
  \label{fig:merged_sets}
\end{figure}


\textbf{Validation with the pivot version objects.}
Algorithm \ref{alg:successors_validation} shows our detailed implementation of the pseudo-code shown in Algorithm \ref{alg:successors_validation_pseudo}. 
In (1), protocols fetch the pivot version objects for all $x_j$ in $ws_j$.
(2) is the validation of ST-Rule by comparing epoch numbers.
(3) and (4) are similar to (C) and (D) in Algorithm \ref{alg:successors_validation_pseudo} but present two cases of false positives.
First, hash collisions incur false positives.
When a hash function $h$ assigns data items $y$ and $z$ into the same slot, we may compare version numbers for different data items $x$ and $y$ and it incurs unnecessary aborts.
The other case of false positives is caused by 4-bits integer truncation of mRS and mWS.
When a version number in $rs_j$ or $ws_j$ is larger than the upper bound of 4-bits integers, we cannot compare the version number correctly.
Then we conclude that MVSG might not be acyclic, and thus NWR-extended protocols do not commit $t_j$ with $\ll^{NWR}$.


\begin{algorithm}[t]
  \caption{validations of $successors_j$ with false positives, where $<_v \in \ll^{NWR}$}  \label{alg:successors_validation}
  \begin{algorithmic}
    \Require{$t_j$}

    \ForAll{$x_j$ in $ws_j$}
    \State{s := get\_the\_pivot\_version\_objects($x$)}
    \Comment{(1)}

    \State %CRLF
    \If{s.epoch $\ne$ $t_j$'s epoch}
    \State %CRLF
    \Return{ST-Rule does not satisfied}
    \Comment{(2)} % $t_j \to ..., \WR{} t_j$
    \EndIf


    \State %CRLF
    % w-r
    \ForAll{$y_m$ in s.mWS}
    \If{$z_n \in rs_j$ and $h(y) = h(z)$}
    \If{$y_m \leq z_n$ or $(2^4-1) \leq z_n$}
    \Comment{(3)} % $t_j \to ..., \WR{} t_j$
    \State %CRLF
    \Return{MVSG may not be acyclic}
    \EndIf
    \EndIf
    \EndFor

    \State %CRLF
    % rw
    \ForAll{$y_g$ in s.mRS}
    \If{$z_j$ $\in ws_j$ and $h(y) = h(z)$}
    \If{$y_g < z_j$ or $(2^4-1) \leq z_j$}
    \Comment{(4)} % $T_j \to ..., \VORW{} T_j$
    \State %CRLF
    \Return{MVSG may not be acyclic}
    \EndIf
    \EndIf
    \EndFor
    \EndFor
    \State{} % CRLF

    \Return{MVSG is acyclic}
  \end{algorithmic}
\end{algorithm}


\subsection{Detailed control flow}
\label{sec:mergedsets_update}

%As we have discussed previously, the pivot version objects are used for the generation of $\ll^{NWR}$ and the validation of the correctness.
Algorithm \ref{alg:NWR_updating_ds} shows the details of the control flow.
In (1), we update mRS for all $rs_j$.
% 現状，abortするときも更新している．．．
% all-newer or all-olderのときは更新しなくてよい (証明がないから書けない)
In (2), we check SR-Rule and ST-Rule of both $overwriters_j$ and $successors_j$.
When some validation fails, NWR-extended protocols quit to validate $\ll^{NWR}$ and then delegate the control flow to baseline protocols to determine $t_j$'s termination operation.
(3) indicates the case when $t_j$ performs the first blind-write $w_j(x_j)$ in the current epoch.
In this case, NWR-extended protocols update all four fields of the pivot version object of $x$ to $x_{pv} = x_j$.
We reset the version number, mRS, and mWS at this time; we update $x_{pv} = 1$, the first pivot version of this epoch.
%mRS and mWS can also reset since there does not exist a committed transaction $t_k$ reachable from $t_j$.
In (4), $t_j$ must update mRS and mWS since at this time $x_{pv}$ is replaced with $t_j$ and thus subsequent transactions need to validate SR-Rule with $t_j$.
It is unnecessary to update both the epoch and the pivot version fields.
% TODO ここはt_jが新たなpivot versionになっている.なぜunnecessaryなのか書くとめっちゃ長い
%At this time $x_{pv}$ is replaced as $x_{pv} = x_j$ but it is unnecessary to update both epoch and the pivot version.
%Since the validation has succeeded, the epoch field always stores $t_j$'s epoch.
%The pivot version is TODO%%

Throughout the control flow, we must access the pivot version objects with the following invariants: 1) both epoch and PV field keeps the information of $t_{pv}$ and must be updated together, and 2) mRS and mWS store merged footprints for all $\{t_{pv}\} \cup RN(t_{pv})$.
When some fields hold inconsistent information, validations may be passed illegally.
The pivot version objects' 128-bits data layout enables us to preserve these invariants with lock-free fashion.
At the beginning of the commit protocol, NWR-extended protocols copy all pivot version objects to another location.
After validation and modification, we call atomic operations such as CAS or DCAS to update all fields atomically.
When CAS or DCAS has failed, we retry the commit protocol from the beginning.


\begin{algorithm}[t]
  \caption{Control flow of NWR-extended protocols}
  \label{alg:NWR_updating_ds}
  \begin{algorithmic}
    \Require{$t_j$}

    \State{\textit{\# Begin atomic section}}
    \ForAll{$x_i$ in $rs_j$}
    \State{s := get\_the\_pivot\_version\_objects(x)}
    \If{s.epoch is the current epoch}
    \ForAll{$y_k$ in mRS}
    \If{$h(x) = h(y)$ and $x_i < y_k$}
    \State{mRS[$h(x)$] := $x_i$}
    \Comment{(1)} % RS update. これはfalse positivenesすぎる(abortするときもやってる)
    \EndIf
    \EndFor
    \EndIf
    \EndFor
    \State

    \ForAll{$x_j$ in $ws_j$}
    \State{s := get\_the\_pivot\_version\_objects(x)}
    \State %CRLF

    \If{validation of $overwriters_j$ or $successors_j$ fail}
      \If{baseline protocols determine $a_j$}
      \Comment{(2)} % Fail
        \State{}
        \Return{abort}
      \EndIf
    \EndIf

    \If{s.epoch is the current epoch}
    \If{$w_j(x_j)$ is the first blind-write in s.epoch}
    \State{s.PV := $x_j$}
    \Comment{(3)} % ST-Rule
    \State{s.epoch := $t_j$.epoch}
    \State{init s.mRS with $rs_j$}
    \State{init s.mWS with $ws_j$}
    \Else
    \Comment{(4)} % SR-Rule
    \ForAll{$y_k$ in s.mRS}
    \If{$z_i \in rs_j$ and $h(y) = h(z)$}
    \If{$z_i < y_k$}
    \State{s.mRS[$h(y)$] := $z_i$}
    \EndIf
    \EndIf
    \EndFor

    \ForAll{$y_k$ in s.mWS}
    \If{$z_j \in ws_j$ and $h(y) = h(z)$}
    \If{$z_j < y_k$}
    \State{s.mWS[$h(y)$] := $z_j$}
    \EndIf
    \EndIf
    \EndFor
    \EndIf
    \EndIf
    \EndFor
    \State{\textit{\# End atomic section}}
    \State %CRLF
    \State{}
    \Return{commit}
    \Comment{all $w_j(x_j)$ in $t_j$ are omittable} % SR-Rule

  \end{algorithmic}
\end{algorithm}




==> IWR-paper copy/tex/introduction.tex <==
\section{Introduction}
Thanks to hundreds of CPU cores and terabytes of RAM on the market, DBMS’s performance bottleneck has shifted from storage I/O to the concurrent processing \cite{Harizopoulos2008OLTPThere}, and thus concurrency control protocols are the key to scaling DBMS performance.
They efficiently interleave read and write operations in transactions; however, they occasionally restrict concurrency by using coordination such as exclusive locking.
Minimizing the number of lockings is a notoriously difficult problem.
Although lockings incurs serious performance penalties, concurrency control protocols cannot avoid to use lockings for preserving \textit{strict serializability} \cite{Herlihy1990Linearizability:Objects} and \textit{recoverability} \cite{Hadzilacos1988ASystems}, the important correctness properties of DBMS.
A number of studies \cite{Lim2017Cicada:Transactions,Kim2016Ermia:Workloads, Yu2016Tictoc:Control,Wang2017EfficientlySerializable,Tu2013SpeedyDatabases,Durner2019NoFalseNegatives,Ding2018ImprovingOptimistic} have addressed this trade-off and succeeded in reducing the number of lockings for read contentions, especially on current industrial standard benchmarks (e.g., TPC-C).

However, recent protocols suffer from emerging workloads on IoT applications and cloud services since their workloads exhibit tremendous write contentions; they frequently collect data from various sources outside DBMS such as sensors, servers, browsers, and mobile devices, and they blindly update shared states simultaneously.
Write contentions in such workloads severely limit the scalability on multi-core processors.
This is because common concurrency control protocols use one exclusive locking per one write operation, and process contended transactions as serial execution.
In fact, it has been known that the performance of recent protocols degrades as the level of write contention increases \cite{Wu2017AnControl, Yu2014StaringCores, Kim2016Ermia:Workloads, Fan:2019:OVG:3342263.3360357}.

Is it possible to reduce the number of lockings for write contentions?
The answer is \textbf{yes}; we show the answer to the question in this paper.
For an intuitive understanding of our approach, we revisit the Thomas write rule (TWR) \cite{Thomas1977ABases} proposed in 1977.
With TWR, we can execute multiple write operations with a single locking.
TWR is a well-known but antiquated optimization rule for the single-version timestamp ordering (T/O) protocol.
If a write operation encounters another one that has a larger timestamp, TWR regards the former is obsolete and \textit{``omittable''}; the execution and locking of the former are unnecessary.
%Only the latter is necessary for DBMS since T/O ensures that the other transactions never access the former.
Even when tremendous write operations for the same data item are running concurrently, we need only a single locking for the single operation with the largest timestamp.

The limitations of TWR are, however, widely known.
First, T/O with TWR incurs unacceptable results for users.
This is because T/O with TWR does not ensure both strict serializability and recoverability as the correctness properties.
Second, TWR is not applicable to the other protocols.
The rule of TWR assumes to use per-transaction, totally-ordered, and monotonically-increasing timestamps; however, recent protocols have not always such timestamps.
T/O with TWR is not in the choices of current DBMSs nowadays, and TWR has not been well studied to apply the concept of omittable for recent protocols.

\textbf{Our goal is to construct an easily-applicable rule to omit write operations with preserving the correctness.}
In this paper, we rethink the formal aspects of omittability.
Although TWR is recognized as the rule for the single-version T/O protocol, we analyze it in terms of the theory of multi-version protocols.
The concept of \textit{version orders} \cite{Bernstein1983MultiversionAlgorithms} in multiversion serializability theory is essential to provide both the theoretical analysis and the applicable approach.
For theoretical analysis, version orders enable us to formalize the definition of omittability without the T/O's timestamps.
As a result, we found that an omittable write operation preserves the correctness only if there exists a version order reverse to the operation order.
Version orders also play a crucial role in the applicability.
It derives the idea that any protocol can be extended to omit write operations by \textbf{validating an additional (reverse) version order}.
Generally, concurrency control protocols generate and validate only a single version order, which is tightly coupled to the implementation of each protocol; however, any protocol can in theory generate and validate an arbitrary number of version orders.
Hence, by adding a version order reverse to the operation order, any protocol has the possibility to omit write operations.

Based on the findings, we construct a new rule for any protocol: \textbf{non-visible write rule (NWR)}.
The main idea of NWR is to extend existing protocols to \textbf{NWR-extended protocols}, that validate an additional version order.
If the additional version order is validated and the rules of NWR are satisfied, NWR-extended protocols generate omittable write operations with the guarantee of strict serializability and recoverability.
Our approach is extensible for any protocol since we add the version order and its validation, not depending on any baseline implementation.

To illustrate the effectiveness of our approach, we show three NWR-extended protocols: Silo+NWR \cite{Tu2013SpeedyDatabases}, TicToc+NWR \cite{Yu2016Tictoc:Control}, and MVTO+NWR \cite{Reed1978NamingSystem., Bernstein1982ConcurrencySystems}.
All of our extensions are implemented in the same way; we embed information for the additional validation (the additional version order and read/write sets of committed transactions) for each data item as a 128-bits data structure.
On 64-bits machines with double-word atomic operations, an omittable write operation is executed by a single atomic operation.
Compared to the conventional approach with exclusive lockings, our approach promises surprisingly high concurrency and scalability.
In our experiments, Silo+NWR achieves up to 11x faster than the original Silo under write contended workloads.
Meanwhile, every NWR-extended protocol has comparable performance with the original, even in the other workloads such as TPC-C in which there are no omittable write operations.

The rest of this paper is organized as follows: we rethink and formalize the definition of TWR, and discuss the formal aspects of ``omittable'' write operations (Section \ref{sec:formal_aspects_of_iw}).
We introduce our approach of validating the additional version order for generating omittable write operations and propose NWR, the rule for a version order to preserve the correctness (Section \ref{sec:design_overview}).
%We introduce NWR, a sufficient condition for omitting write operations for any concurrency control protocol (Section \ref{sec:invisiblewriterule}).
We show the implementation detail of the proposed approach (Section \ref{sec:implementation}). 
We examine three NWR-extended protocols and confirm that every extended protocol shows a significant performance gain in write-contended workloads (Section \ref{sec:evaluation}). 


==> IWR-paper copy/tex/invisiblewriterule.tex <==

% ここまで


==> IWR-paper copy/tex/lockfreevs.tex <==
\section{Manipulating MergedSet}
\label{sec:lockfreevs}

Next, we show the details of the implementation of LI-Rule and tracking $successors_j$ for a running transaction $T_j$, by using the data structure described in Appendix \ref{sec:implement}.
Briefly, we use FV and Epoch for LI-Rule, and we use MergedRS and MergedWS for SR-Rule.

As described in Appendix \ref{sec:algorithms}, we need to validate that MVSG is acyclic, by using readsets and writesets for all $T_k \in \{successors_j \cup overwriters_j\}$ and all $T_i \in RN(T_k)$.
We compress these sets into MergedRS and MergedWS to manipulate with lock-free fashion.

\begin{algorithm}[t]
  \caption{Tracking of $successors_j$ with MergedRS and MergedWS}
  \label{alg:successors_validation}
\begin{algorithmic}
   \Require{$T_j$}
   
    \ForAll{$x_j$ in $ws_j$}
       \State{MergedRS, MergedWS := Index.get($x$)}
       \Comment{(1)} % $T_j \to ..., \VORW{} T_j$
       
       \State %CRLF
       % w-r
        \ForAll{$vs(y_k)$ in MergedWS}
           \If{$y_i$ $\in rs_j$ and !$(2^4-1 \leq vs(y_k) \land 2^4-1 \leq vs(y_i))$}
             \Comment{(2)} % $T_j \to ..., \WR{} T_j$
             \If{$vs(y_k) \leq vs(y_i)$}
                \State %CRLF
                \Return{MVSG may be not acyclic}
              \EndIf
           \EndIf
         \EndFor
         
         \State %CRLF
         % rw
        \ForAll{$vs(y_k)$ in MergedRS}
           \If{$y_j$ $\in ws_j$ and !$(2^4-1 \leq vs(y_k) \land 2^4-1 \leq vs(y_j))$}
              \Comment{(3)} % $T_j \to ..., \VORW{} T_j$
              \If{$vs(y_k) < vs(y_j)$}
                \State %CRLF
                \Return{MVSG may be not acyclic}
              \EndIf
           \EndIf
         \EndFor
    \EndFor
    \State{} % CRLF

    \Return{MVSG is acyclic}
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:successors_validation} shows the details of Algorithm \ref{alg:successors_validation_pseudo}, which validates that any edge from any $T_k \in successors_j$ cannot reach into a running transaction $T_j$.
We can reduce the number of loop processing than Algorithm \ref{alg:successors_validation_pseudo} by compressing both readset and writeset.
In (1), our NWR schedulers fetch both readset and writeset for all $T_k$ such that $T_k = T_{FV}$ or $T_k \in RN(T_{FV})$ for a transaction $T_{FV}$ which had written $x_{FV}$.
Because whole the data structure is within 128-bits, We can implement fetching MergedRS and MergedWS with lock-free fashion.
In (2) and (3), we treat the counter saturation.
Necessarily, compressing causes the boundary of counters.
Because each slot of MergedRS and MergedWS has only four-bits, if $vs$ returns the number larger than $2^4-1$, we must treat this case as false-positiveness.
Thus, in this case, we have to decide that MVSG may not be acyclic and $T_j$ cannot
commit with the version order based on the all invisible strategy.

\subsection{Updating The Data Structure}

In this subsection, we show how and when the data structure should be updated.
If validations of SR-Rule or LI-Rule for a running transaction $T_j$ with the version order $\ll$ based on the all invisible strategy has failed,
our NWR schedulers validate the other version order $\ll'$ generated by underlying schedulers.
If the validation with $\ll'$ has also failed, NWR schedulers must abort $T_j$.
Otherwise, our NWR schedulers commit $T_j$ with $\ll'$.
In this case, we must update each field of the data structure of $x$ for all $x_j \in ws_j$ and $x_i \in rs_j$.
Updating the data structure leads to improve commit rate with $\ll$ for subsequent transactions.
For example, if LI-Rule is not satisfied with $\ll$, we can update FVes just like $x_{FV} = x_j$ for all $x_j \in ws_j$ and store the current epoch into the epoch field of the data structure.
At the next time, for a new running transaction $T_j'$, our NWR schedulers validate a version order different with $\ll$; if $T_j$ and $T_j'$ access the same data items, all $x_{FV}$ for all $x_j' \in ws_j'$ are updated.
Besides, if $T_j$ and $T_j'$ is in the same epoch, LI-Rule is always satisfied.
Thus, under this policy, we guarantee that validation failures of LI-Rule happen at most only once for each epoch for each data item.

\begin{algorithm}[t]
  \caption{Updating The data structure}
  \label{alg:NWR_updating_ds}
\begin{algorithmic}
   \Require{$T_j$, Index}
   
    \ForAll{$x_j$ in $ws_j$}
       \State{$vs(x_{FV})$, epoch, MergedRS, MergedWS = Index.get($x$)}
       \State %CRLF
       
       \If{$T_j$.epoch $\ne$ epoch}
        \Comment{(1)} % LI-Rule
            \State{$vs(x_{FV})$ := 1}
            \State{epoch := $T_j$.epoch}
            \State{MergedRS := $rs_j$}
            \State{MergedWS := $ws_j$}
            \State % CRLF
       \Else
        \Comment{(2)} % SR-Rule
            \ForAll{$vs(y_k)$ in MergedRS}
                 \If{$vs(y_k) = 0$ or $vs(y_j) < vs(y_k)$}
                     \State{MergedRS[$h(y)$] := $vs(y_j)$}
                 \EndIf
              \EndFor
               \State %CRLF
               
             \ForAll{$vs(y_k)$ in MergedWS}
                 \If{$vs(y_k) = 0$ or $vs(y_j) < vs(y_k)$}
                     \State{MergedWS[$h(y)$] := $vs(y_j)$}
                 \EndIf
              \EndFor
               \State %CRLF
         \EndIf
      \EndFor
      
     \If{$rs_j \ne \phi$}
         \Comment{(3)} % Read
         
         \State{all-older, all-newer = true}
         \ForAll{$x_k$ in $rs_j$}
             \State{$vs(x_i)$ := Index.get($x$)}
              \If{$vs(x_i) < vs(x_k)$}
                  \State{all-newer = false}
              \Else
                   \State{all-older = false}
              \EndIf
           \EndFor

           \If{all-newer or all-older}
              \Return         
              \Comment{(4)} % Optimization
           \EndIf
                      \State %CRLF
           \ForAll{$x_k$ in $rs_j$}
              \State{MergedRS := Index.get($x$)}
                  \ForAll{$vs(y_i)$ in MergedRS}
                      \If{$y_k$ in $rs_j$}
                          \If{$vs(y_i) = 0$ or $vs(y_k) < vs(y_i)$}
                               \State{MergedRS[$h(y)$] := $vs(y_k)$}
                           \EndIf
                       \EndIf
                 \EndFor
           \EndFor
     \EndIf
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:NWR_updating_ds} shows the updating process of the data structure.
Let $\ll, \ll'$ be a version order generated by collecting FVes (based on all invisible strategy) and a version order generated by underlying schedulers, respectively.
Our NWR schedulers process this algorithm only when a running transaction $T_j$ can commit only with $\ll'$.

In (1), we update all FV, epoch, MergedRS, and MergedWS if LI-Rule is not satisfied with $\ll$.
Thus, some $x_{FV}$ for some $x_j \in ws_j$ is written in the old epoch.
Then we update the data structure of each data item $x$ so as to $x_{FV} = x_j$.
In this case, because FV will be updated, MergedRS and MergedWS have to store the information of $T_j$.
Moreover, we rewind the integer $vs$ of the version $x_j$ just like $vs(x_j) = 1$.
Because LI-Rule prohibits schedulers from reordering transactions across epochs, $vs$ only have to reflect the order of versions which have written in the same epoch.
Thus, we can rewind $vs$ safely and prevent counter saturation of MergedRS and MergedWS.

In (2), we must update MergedRS and MergedWS for all $x_j$ in $ws_j$.
We need to update MergedRS and MergedWS for each transaction which is reachable from $T_{FV}$.
Since our scheduler commits $T_j$ with $\ll'$ and $T_{FV}$ is in the same epoch with $T_j$,
there may exist a path such as $T_{FV} \to ... \to T_j$.

In (3), NWR schedulers must update MergedRS for all $r_j(x_k)$ in $op(T_j)$.
Note that we must update MergedRS only when some $T_{FV}$ has some path to $T_j$.
Thus, for reducing the coordination in read-intensive workload,
we optimize the update processing in read operations.
In (4), we check that all $x_{FV}$ is newer or older than $x_k \in rs_j$.
If it holds, we can skip updating MergedRS because $T_j$ will never be included in the cyclic path of MVSG for all subsequent transactions.
Note that $T_j$ is in the cyclic path if and only if there is some path from some $T_{FV}$ to $T_j$, and there is some path to another $T_{FV}$ from $T_j$.
% NOTE これproofない
Moreover, we can implement further optimization based on this consideration; when $T_j$ must update MergedRS, we can retry $T_j$ to read only good versions older or newer than FVes.
Under this optimization, read-only transactions avoid any updating the data structures.

As has been noted, we implement updating the data structure in the lock-free fashion.
Thus, if we need to update some field in the data structure, we must copy it to another location.
After validation and modification, we call atomic operations such as CAS or DCAS to update all field atomically.
When CAS or DCAS has failed, we must retry this algorithm; copy the data structure once more, and retry validation, modification, and calling atomic operations.


==> IWR-paper copy/tex/omittable.tex <==
\section{Omittable Write Operations}
\label{sec:formal_aspects_of_iw}
In this section, we first rethink the formal aspects of omittable write operations allowed by TWR.
%We then formalize when a write operation is omittable with preserving the correctness.
TWR does not have any formal definitions and propositions for the correctness but explained as follows \cite{Bernstein:2009:PTP:1208930}:%We then construct a new rule named NWR for any protocol that ensures the correctness with omittable write operations and compare it with TWR. 

\begin{figure*}[t]
  \centerline{
    \subfloat[$x_1 <_v x_3$. Everyone allows]{
      \includegraphics[clip, width=0.25\textwidth]{img/csr_wrw.pdf}
    }
    \hfill
    \subfloat[$x_1 <_v x_3$. TWR allows]{
      \includegraphics[clip,width=0.25\textwidth]{img/twr_wrw.pdf}
    }
    \hfill
    \subfloat[$x_1 <_v x_3$. TWR forbids]{
      \includegraphics[clip,width=0.25\textwidth]{img/mvsr_wrw.pdf}
    }
    \hfill
    \subfloat[$x_3 <_v x_1$. TWR forbids]{
      \includegraphics[clip,width=0.25\textwidth]{img/mvsr_wrw2.pdf}
    }
  }
  \caption{Schedules with version orders. All schedules are strict serializable. Horizontal lines of each transaction indicate the transaction's lifetime. Transactions begin at the start point of their line. (b-d) include an omittable write operation $w_1(x_1)$, $w_1(x_1)$, and $w_3(x_3)$, respectively. Operations painted as trash boxes are omitted. TWR can omit $w_1(x_1)$ in the case of (b), but reject the cases (c) and (d).}
  \label{fig:wrw_optim}
\end{figure*}

\begin{quote}
If an update to data item $x$ arrives at a replica, and the update's timestamp is larger than $x$'s timestamp at the replica, then the update is applied and $x$'s timestamp is replaced by the update's timestamp.
Otherwise, the update is discarded.
...
And eventually, each data item $x$ has the same value at all replicas, because at every replica, the update to $x$ with the largest timestamp is the last one that actually was applied
\end{quote}
where the term ``replica'' means a thread or a machine node.
Here we see that a write operation with the lower timestamp is discarded.
It is based on the fact that the other transactions will never read the discarded write operations; in T/O, a transaction reads the current versions that have the maximal timestamp for each data item.
Therefore, it is unnecessary to apply discarded write operations.
The necessity of applying write operations in TWR derives an essential observation of what is \textit{omittable}:

\begin{observation}
  \label{observation:lazy}
  Execution of a write operation $w_i(x_i)$ can be delayed until a read operation $r_j(x_i)$ arrives.
\end{observation}

%Since the definition of multiversion schedules does not restrict when protocols must execute each write operation, protocols can delay execution of write operations until just before an associated read operation comes.
% NOTE: もともとここに↑が書かれていた．「理論的には，いつwriteを実行する，という定義がないわけだから，スケジュールには存在するが実行は遅延されている，という状況も解釈可能だろう」という感じ．
% これはAxiomとして書かれていたころは必要だったと思う．いまはobservationにしてしまったので，observationの理論的補強を書くのは違和感．

Clearly, T/O with TWR utilizes this observation.
Since T/O's read protocol guarantees that discarded versions are never be read, TWR safely postpones executions of write operations indefinitely.
Throughout the paper, we define ``omitting'' as indefinitely delaying execution of an operation.
Based on this observation, we now define an omittable write operation without the concept of timestamps:

\begin{definition}[Omittable]
  \label{def:omittable}
  A write operation $w_j(x_j)$ is \textbf{omittable} if there \textbf{always} does not exist $t_i$ such that $r_i(x_j)$ is in $t_i$.
\end{definition}

Definition \ref{def:omittable} states that any protocol can generate omittable write operations since the timestamps are no longer needed.
For a version $x_j$, if there is the guarantee of non-visibility of $x_j$, we can omit $w_j(x_j)$.
In fact, this guarantee is provided by simply omitting $w_j(x_j)$ without lockings, updating timestamps, or any coordination among the other transactions.
Since omitting does not store any footprints of $x_j$, subsequent transactions cannot know $x_j$'s existence.
%The problem is the correctness of the resulting schedules.

Next, we consider the correctness for the generated schedules.
After omitting a write operation, does a strictly serializable protocol even keep this property?
The answer is derived from version orders and concurrency of transactions.
Remind that a schedule is serializable iff there exists a version order which makes the MVSG acyclic, and it is strictly serializable iff there does not exist reordering of operations or versions among non-concurrent transactions.
Hence, if a protocol finds out a version order and validates the concurrency of transactions, the generated schedules are still strictly serializable.
We later show the formal condition and validation for a version order in Section \ref{sec:invisiblewriterule}.
Note that omittable write operations do not affect recoverability; recoverability is violated only when a committed transaction read a version written by a non-committed transaction \cite{Hadzilacos1988ASystems}.

\subsection{Discussion}

We now rethink TWR in terms of version orders and reveal that TWR is the too restrictive rule.
%We can in theory omit more write operations with the correctness.
Figure \ref{fig:wrw_optim} depicts four schedules and version orders.
Notice that all schedules are strictly serializable since all MVSGs with illustrated version orders are acyclic, and all transactions are concurrent.
In Figure \ref{fig:wrw_optim}, (b-d) include an omitted operation, but (a) does not.
We assume subscripts represent timestamps of T/O, and thus T/O with TWR allows omitting only in the case of (b).
In (c), T/O must abort $t_1$ since the read-timestamp of $x_3$ has already updated.
In (d), T/O must execute $w_3(x_3)$ since timestamps indicate $t_1 < t_3$; thus $t_3$ must execute $x_3$ as the latest version of $x$ and $x_3$ does not have non-visible property.
It should be pointed out that (a) and (d) show the completely same schedules, and the only difference is the version orders.
In these schedules, we can in theory omit $w_3(x_3)$; however, the existing lock-based or timestamp-based protocols \cite{Bernstein1987ConcurrencySystems,Tu2013SpeedyDatabases,Lim2017Cicada:Transactions, Larson2011High-performanceDatabases} always execute $w_3(x_3)$ as the latest (visible) version of $x$ since their version orders are generated based on the locking order or the timestamp order.
The tight coupling between version order generation and protocol implementation is the current limitation for improving the performance of write operations.

% TODO
% ここにSec.5ぶちこむ？
% T/O with TWRは，タイムスタンプによってserializabilityを保証していたが， STとRCについては保証されていなかった．
% 我々は，ここで，omittalbe write operations with strict serializability and recoverabilityの定義を，NWRとして示す．
% Sec. 4 



% \textbf{Class 1: unnecessary aborts.}
% In (c), T/O must abort $t_1$ since the read operation $r_2(x_3)$ has already read $x_3$.
% T/O forces transactions to process read and write operations in the timestamp order.
% Therefore, in (c), if $t_1$ was committed, $t_2$ should have accessed $x_1$; however, $t_2$ already read $x_3$ and committed.
% T/O gives \textit{read-timestamp} for each version to validate and abort such transaction $t_1$.


% \textbf{Class 2: impossible version orders.}
% In (d), T/O with TWR must execute $w_3(x_3)$ since T/O cannot ensure the non-visible property of $x_3$. 
% Since the timestamp indicates $x_1 < x_3$, other subsequent transactions will may read $x_3$.


% \textbf{TWR and strict serializability.}
% It is known that all threads or nodes get the same versions eventually with TWR \cite{Thomas1977ABases}; however, it is unclear that an eventual schedule is strictly serializable.
% With the theory of MVSR, we can easily give a counterexample.
% Let $S = w_j(x_j)c_jw_k(x_k)$ be a schedule.
% Clearly $t_j$ is not concurrent with $t_k$.
% A version order for the data item $x$ which includes $x_k <_v x_j$ breaks strict serializability, since $t_k$ writes the older version than $t_j$'s one.
% However, T/O with TWR may generate such an invalid version order when the order of timestamp $TS$ indicates $TS(k) < TS(j)$.
% Hence, T/O with TWR is serializable but not strictly serializable.



==> IWR-paper copy/tex/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\begin{table}[t]
  \small
  \begin{tabular}{|c|l|} \hline
      Symbol & Definition \\ \hline \hline
    $D$ & a set of distinct finite data items ($x, y, z,...$) \\
    $t_i$ & $i$-th transaction. an ordered set of operations \\
    $x_i$ & a version of a data item $x$\\
    $w_i(x_i)$ & a write operation. $t_i$ writes a version $x_i$ \\
    $r_i(x_j)$ & a read operation. $t_i$ reads $x_j$ \\
    $c_i$ & a termination operation which commits $t_i$ \\
    $a_i$ & a termination operation which aborts $t_i$ \\
    $rs_i$ & a set of versions read by $t_i$ \\
    $ws_i$ & a set of versions written by $t_i$ \\
    $\{x\}$ & a set of versions of a data item $x$ \\
    $S$ & a schedule. \footnotemark[1] \\
    $CP(S)$ & returns committed projection of $S$ \\
    $trans(S)$ & returns a set of transactions in $S$ \\
    $\ll$ & a version order for a schedule. \footnotemark[2] \\
    \hline
  \end{tabular}
  \caption{Definitions of main symbols}
  \label{tab:symbols}
\end{table}

\footnotetext[1]{
     A schedule is a pair of operations and $<_s$ where $<_s$ is an order for all pairs of operations from distinct transactions that access the same data item and have at least one write operation \cite{Weikum2001TransactionalRecovery}.
}
\footnotetext[2]{
  A version order for $x$ is any non-reflexive and total ordering of $\{x\}$.
  A version order for a schedule is the union of all version order for data items written by operations in the schedule
  \cite{Weikum2001TransactionalRecovery}.
}

In this paper, we mainly use the notations defined by Weikum and Vossen \cite{Weikum2001TransactionalRecovery}.
Table \ref{tab:symbols} shows definitions of main symbols.
Note that $rs_i$ (read set) and $ws_i$ (write set) are available for all protocols by adding the corresponding sets.
% TODO これいるのか？ 川島先生曰くディフェンスのために必要らしいが，自明に思える
We use symbols and notations of multi-version concurrency control throughout this paper.
Without loss of generality, we can assume that all data items have multiple versions, and all schedules are multi-version schedules \cite{Papadimitriou1986TheControl, Weikum2001TransactionalRecovery, Bernstein1987ConcurrencySystems}.

We consider \textbf{the correctness} of DBMS in the aspects of strict serializability \cite{Herlihy1990Linearizability:Objects} and recoverability \cite{Hadzilacos1988ASystems}.
Strictly serializable protocols always generate schedules equivalent to some serial executions in a single thread on a single machine.
Recoverable protocols ensure that DBMS can always be recovered without any dirty-read \cite{10.1145/223784.223785} anomaly whenever some aborts or crashes happen.
In the following, we explain the details of strict serializability.
The formal definition of recoverability is given in Appendix \ref{sec:proof}. 

\subsection{Serializability and its graph}
\label{sec:def_of_mvsg}
To explain strict serializability, we first introduce serializability.
For a schedule $S$, multiversion view serializability (MVSR) \cite{Papadimitriou1982OnVersions} is defined that $S$ is serializable iff $S$ is \textit{view equivalent} with some serial schedules.
To obtain the view-equivalent serial schedules, Bernstein et al. proposed the multiversion serialization graph (MVSG) \cite{Bernstein1983MultiversionAlgorithms} and prove that $S$ is MVSR iff there exists acyclic MVSG.
An MVSG is generated based on a schedule $S$ and a version order $\ll$.
``$x_i <_v x_j$'' denotes that a version $x_i$ precedes another version $x_j$ in $\ll$.
For given $S$ and $\ll$, an $MVSG(S, \ll)$ has nodes for $trans(CP(S))$ and edges as the followings:
for distinct operations $w_j(x_j)$, $r_i(x_j)$, and $w_k(x_k)$ where $t_i \ne t_k$ and $t_j, t_i, t_k$ in $trans(CP(S))$,
\begin{itemize}
  \setlength\itemsep{0.14em}
\item $t_j \WR{} t_i$
\item If $x_j <_v x_k$  then $t_i \VORW{} t_k$
\item If $x_j >_v x_k$  then $t_k \VOWW{} t_j$
\end{itemize}
We denote $\WR{}$, $\VORW{}$, and $\VOWW{}$ as edges of MVSG and $\to$ as any of edges.
%There are two types of version order: a version order for a data item, and a version order for a schedule.
%The version order for a data item $x$ is any non-reflexive and total ordering of $\{x\}$.
%The version order for a schedule $S$ is the union of the version orders for all data items in $D$.
Note that all serializable protocols have their version orders generated by their implementation, such as lockings, timestamps, or transaction ids.
For $MVSG(S, \ll)$, we define a function $RN(t_i)$ which accepts a transaction $t_i$ in $trans(CP(S))$ and returns a set of transactions that includes reachable transactions from $t_i$ on MVSG.

\subsection{Strict serializability}
Strict serializability \cite{Herlihy1990Linearizability:Objects, Fan:2019:OVG:3342263.3360357,10.14778/3342263.3342647} is the property of serializable schedules.
Intuitively, it is the wall-clock ordering constraints among transactions.
In general, distributed concurrency control protocols promise strict serializability for preventing \textit{stale reads}, that read too old versions.
This property is also essential for non-distributed protocols to prevent \textit{stale writes}, that write too old versions.
For instance, a serializable protocol allows all transactions to read and write into an arbitrary version.
A transaction can always read the initial values written by $t_0$ even if there exist some newer versions, and also can always write older versions than the initial values such as $x_j <_v x_0$.
Even if several years may have passed after the initialization of DBMS, not strictly serializable protocols allow such unacceptable results.
To satisfy strict serializability, we must forbid protocols from reordering among operations or versions when these transactions are not concurrent.
A more formal definition of this property is described in Appendix \ref{sec:proof}. 



==> IWR-paper copy/tex/proof.tex <==
\section{Formal Proof}
\label{sec:proof}


We need the following lemmas to prove Theorem \ref{theo:NWR_is_correct}.
Each lemma corresponds to serializability, strict serializability, and recoverability, respectively.

\begin{lemma}[Serializable]
\label{theo:NWR_is_sr}
For a triple $(S, \ll, t_j)$ which satisfies NWR,
$S \cup \{c_j\}$ is serializable.
\end{lemma}

\begin{proof}
To prove by contradiction,
we assume that $MVSG(S \cup \{c_j\}, \ll^{NWR})$ for any $\ll^{NWR}$ is not acyclic.
By PV-Rule, $MVSG(S, \ll)$ and $MVSG(S, \ll^{NWR})$ are isomorphic.
To form the cycle, there exists some paths $t_j \to t_k \to ..., \to t_j$ for some $t_k$.
By SR-Rule, there exists no edge $t_k \to t_j$ for all $t_k \in RN(t_j)$.
It implies the contradiction.
\end{proof}
% By the definition of MVSG \cite{Bernstein1987ConcurrencySystems,Bernstein1983MultiversionAlgorithms}, it is enough to consider the following three cases of the edge which has $T_j$ as a source:
% \begin{enumerate}

% \item  Case 1: $T_j \stackrel{wr}{\to} ..., \to T_j$.
% By RC-Rule, all transaction $T_i \in trans(CP(S))$ do not read any data item $x_j \in ws_j$.
% Thus, there exists no edge from $T_j$ such that $T_j \WR{} ..., \to T_j$.

% \item  Case 2: $T_j \stackrel{\ll(rw)}{\to} ..., \to T_j$.
% By definition of MVSG, an edge $T_j \VORW{} T_k$ is added into $MVSG(S', \ll^{NWR})$ if $\exists x_k\exists x_i(x_k \in ws_k \land x_i \in rs_j \land x_i <_v x_k)$ where $<_v \in \ll^{NWR}$ holds.
% $overwriters_j$ includes all $T_k$.
% Thus, by SR-Rule, there exists no edge from $T_j$ such that $T_j \VORW{} ..., \to T_j$. 

% \item  Case 3: $T_j \stackrel{\ll(ww)}{\to} ..., \to T_j$.
% By definition of MVSG, an edge $T_j \VOWW{} T_k$ is added into $MVSG(S', \ll^{NWR})$ if $\exists x_k \exists x_j \exists T_g(x_k \in ws_k \land x_j \in ws_j \land x_j <_v x_k \land T_g \in trans(CP(S')) \land x_k \in rs_g)$ where $<_v \in \ll^{NWR}$ holds.
% $successors_j$ includes all $T_k$.
% Thus, by SR-Rule, there exists no edge from $T_j$ such that $T_j \VOWW{} ..., \to T_j$. 
% \end{enumerate}
% Thus, $MVSG(S', \ll^{NWR})$ is acyclic.


\textbf{Strict serializability.}
The definition of strict serializability is following \cite{Herlihy1990Linearizability:Objects}:
\begin{quote}
A history is serializable if it is equivalent to one in which transactions appear to execute sequentially, i.e., without interleaving. A (partial) precedence order can be defined on non-overlapping pairs of transactions in the obvious way. A history is strictly serializable if the transactions’ order in the sequential history is compatible with their precedence order. 
\end{quote}
As has been noted, a schedule $S$ is serializable iff there exists a version order $\ll$ such that $MVSG(S, \ll)$ is acyclic.
Strict serializability is the condition of the order $M$, a total order of transactions generated by topologically-sorting of acyclic MVSG.
We define the formal definition\footnotemark[3] of strict serializability for a schedule $S$ and a total order of transactions $M$ as following:
$\forall t_i \forall t_k \forall p \forall q(((p \in t_i \land q \in t_k) \land p <_S q) \Rightarrow t_i <_M t_k)$ where $<_M$ in $M$ and $<_S$ in $S$.

\begin{lemma}[Strictly serializable]
\label{theo:linearizable}
For a triple $(S, \ll, t_j)$ which satisfies NWR,
$S \cup \{c_j\}$ is strictly serializable.
\end{lemma}

\begin{proof}
By Lemma \ref{theo:NWR_is_sr}, $MVSG(S \cup \{c_j\}, \ll^{NWR})$ is acyclic for some $\ll^{NWR}$.
Let $M$ be a total order of $trans(CP(S \cup \{c_j\}))$ generated by commit-ordered first topological-sorting for MVSG.
To prove by contradiction, we assume that $S\cup \{c_j\}$ is not strictly serializable.
By assumption, there exists some $t_i$ in $trans(CP(S))$ such that (a) $\forall p \forall q(((p \in t_i \land q \in t_j) \land p <_S q)$ but (b) $t_j <_M t_i$.
(b) implies that MVSG includes the path $\{t_j \to ..., \to t_i\}$.
However, by ST-Rule, there exists some $q$ in $t_j$ such that $q <_S c_k$ for all reachable transactions $t_k$ in $RN(t_j)$.
That is, if (a) holds for some transaction $t_i$, (b) does not hold; there always exists $q$ in $t_j$ such that $q <_S c_i$.
It implies the contradiction.
\end{proof}

\footnotetext[3]{We define that the operation order in a given schedule reflects the wall-clock order.}

\textbf{Recoverability.}
The formal definition of recoverability is the following \cite{Weikum2001TransactionalRecovery}: 
$$\forall t_i \forall t_j ((t_i, t_j \in trans(S) \land t_i \ne t_j) \Rightarrow (r_j(x_i) \in t_j \Rightarrow c_i <_S c_j)$$
\begin{lemma}[Recoverable]
    \label{theo:recoverable}
For a triple $(S, \ll, t_j)$ which satisfies NWR,
$S \cup \{c_j\}$ is recoverable.
\end{lemma}
\begin{proof}
To prove by contradiction, we assume that $S\cup \{c_j\}$ is not recoverable.
Since $S$ is recoverable, there exists $x_i$ such that $c_i,a_i \notin S$ and $x_i$ in $rs_j$.
By RC-Rule, it does not hold.
\end{proof}


Finally, we now prove Theorem \ref{theo:NWR_is_correct}.
\begin{proof}
    \label{proof:NWR_is_correct}
    By Lemma \ref{theo:linearizable}, $S \cup \{c_j\}$ is strictly serializable.
    By Lemma \ref{theo:recoverable}, $S \cup \{c_j\}$ is recoverable.
\end{proof}


==> IWR-paper copy/tex/relatedwork.tex <==
\section{Related Work}

% 日本語
% Thomas write rule.
% Section で述べたように，TWRは書き込みをomitすることをT/Oに許容しているルールである．
% NWRにくらべ，TWRは2つの点で制限的であり，この2つの点はともにT/Oの実装にあるtimestampに起因する．
% まず，TWRはversion orderを一つしか検証できない．
% T/Oが生成したtimestamp based version orderに基づいて，omittableかどうかを検証している．
% 次に，TWRはtimestampが大きいwrite opsをomitできない．
% Axiom 1で示した通り，readされておらず，version orderが最新でないならば，strict SRとRCを満たしてomitできる可能性がある．そのようなケースでも，TWRはomitを許容しない．

% Deterministic database.
% 他のomitの例としては，Deterministic databaseにおける例がある．
% deterministic databaseにおけるomitは...流用
% NWRに比較すると，この例はあまりformalizeされているとはいえないが，いくつか共通点がある．
% DTのcentral schedulerによってgroupされたトランザクションをconcurrentとみなしていること．
% また，readされないことが保証されるwriteを，blind writeで上書きすることだ．
% DTには，NWRにくらべ秀でた点がある．
% それは，epoch内のすべてのトランザクションのRS/WSを処理できるため，
% ある一つのblind updateだけを残して，他のすべてのwriteをomitできるということだ．
% NWR-extended protocolsはnon-deterministic protocolsであるため，そのようなblind writeが同一epochにrequestされるということがわからない．
% よって，同一epoch内で複数のwrite opsを実行してしまう．
% しかし，NWRの定義は，deterministicにも non-deterministicにも有効である．
% deterministicがscalability issueを抱えている\ref{}ワークロードや状況では，
% 我々のアプローチはより汎用的かつ効率的に機能するだろう．

% MVSR schedulers.
% 多くのmulti-version concurrency control protocolsといわれるプロトコルは，MVSR，またの名を1-copy serializabilityを満たすよう設計されている．
% それらは，複数のversionを保持して，そこからプロトコルによって決められたversionを読み出す．
% しかし，version orderを複数検証するという我々のアプローチは類を見ない．
% その理由は，計算量にある．
% あるSchedule においてversion orderを全探索してMVSRかどうかを判定するという決定問題は，， NP-Completeに属する．
% よって，通例では，プロトコルがただ一つ，version orderの生成方法を決定することで計算量を削減している．
% 我々は，ここに，Section で示した PV-Ruleを加えたVersino orderを追加で検証することで，書き込みの最適化を達成した．
% PV-Ruleは非常に効率的に計算量を削減している．ST-RuleとSR-Ruleの判定が，running tjを用いて作るMVSGの部分グラフの問題に帰着できるからだ．
% しかし，Strict SRとRCを満たす"必要十分条件" を考えたとき，PV-Ruleは不要である．
% すべてのversionの順序を組み換えることを許容すれば，running tjをよりomittableにできるかもしれないが，我々はNWR-extended protocolの実用的な実装のため，このPV-Ruleを追加している．

\textbf{Thomas Write Rule.}
As we have been discussed in Section \ref{sec:formal_aspects_of_iw}, TWR allows T/O to omit some write operations.
Compared to NWR, the rule of TWR is more restrictive since TWR requires T/O's timestamps.
TWR validates only a single version order generated by the timestamps and allows omitting only when the timestamp order is satisfied with the rule of TWR.
NWR is the more elastic rule.
It allows any protocol to validate any number of version orders, and it does not depend on any baseline implementation.

\textbf{Lazy transaction execution.} % TODO Another exampleって言い回しあり？
Another example of the protocol which allows generating omittable write operations is in deterministic databases \cite{Ren2014AnSystems,Thomson2012Calvin:Systems}.
Deterministic databases adopt the centralized approach of concurrency control; centralized transaction managers collect transactions and separate them into some batches.
Faleiro et al. \cite{Faleiro2014LazySystems} proposed the approach of \textit{lazy transaction execution}.
It enables deterministic databases to omit some write operations.
By delaying the execution of write operations, deterministic databases execute only blind updates, which writes the latest version in each batch.
Lazy transaction execution makes other write operations omittable.
This approach is similar to our approach of NWR-extended protocols, in terms of grouping transactions; both approaches separate transactions and execute only the latest versions. 
Compared to lazy evaluation, the rule of NWR and the approach of validating the additional version order is more applicable for any protocol, since the rule of NWR does not require the centralized transaction manager.
NWR is useful for both deterministic and non-deterministic databases.

\textbf{Multiversion concurrency control protocols.}
Multiversion concurrency control (MVCC) protocols \cite{Lim2017Cicada:Transactions, Fekete2005MakingSerializable, Larson2011High-performanceDatabases} can hold multiple versions for each data item.
Multiversion read avoids the highly abort rates of single-version protocols, especially in workloads that include long-transactions \cite{Yu2014StaringCores,Wu2017AnControl,Kim2016Ermia:Workloads}.
MVSR is widely used to guarantee the correctness of MVCC, and thus all MVCC protocols can in theory generate multiple version orders.
However, existing multiversion protocols \cite{Larson2011High-performanceDatabases,Lim2017Cicada:Transactions,Kim2016Ermia:Workloads,Ports2012SerializablePostgreSQL,Kemper2011HyPer:Snapshots} generate only a single version order.
This is because the computational cost of the decision problem to find a suitable version order from all possible orders is NP-Complete \cite{Bernstein1983MultiversionAlgorithms,Papadimitriou1982OnVersions}.
Furthermore, the approach of validating multiple version orders requests protocols to verify multiple MVSGes, and it causes enormous overheads. 
NWR and NWR-extended protocols efficiently reduce the computational cost of validating multiple version orders.
NWR-extended protocols add only a single version order, which is ideal for omitting; thus, they validate only two MVSGes.
Besides, PV-Rule of NWR defines that the two MVSGes are isomorphic if a running transaction $t_j$ aborts.
Therefore, additional validation is required only for a connected subgraph which includes $t_j$.
NWR-extended protocols achieve to validate multiple version orders efficiently; they maintain only a single version order and validate two almost the same MVSGes. 


==> IWR-paper copy/tex/versionorders.tex <==
\section{Extending Conventional Schedulers To NWR schedulers}
\label{sec:vmvo}

We observed in Section \ref{sec:invisiblewriterule} that NWR schedulers can generate a pair of a schedule and a version order, which includes IW.
In this section, we describe 1) which version order generated by NWR schedulers is useful for improving throughput, and 2) how to extend conventional schedulers to NWR.

\subsection{All Invisible Strategy}
\label{sec:mivo}

To fully optimize write operations, we introduce the \textbf{All Invisible Strategy} for generating version orders.
Let a schedule $S$ and a running transaction $T_j$ such that $c_j, a_j \notin S$.
The version order $\ll$ based on the all invisible strategy satisfies $\forall w_j(x_j) \exists x_k (w_j(x_j) \in op(T_j) \Rightarrow (x_k \in \{x\} \land x_j <_v x_k))$.
That is, all write operations of $T_j$ always become IW operations when schedulers generate $S'$ such that $c_j \in S'$.
By omitting all write operations, the version order based on the all invisible strategy maximizes the performance of write operations.

However, generating the version order based on the all invisible strategy may worse for the performance.
Because MVSGes depend on version orders, commit ratio of schedule depends on version orders.
Thus, if we extend a conventional scheduler to an NWR scheduler, we cannot guarantee that the performance of the NWR scheduler is better or equal to the performance of the underlying scheduler, even in the same workload.

\subsection{Validating Multiple Version Orders}

To keep the commit rate of underlying schedulers and to improve the performance of write operations, we introduce \textbf{Validating Multiple Version Orders (VMVO)}.
In contrast with conventional approaches, maintain and validate the only one version order, VMVO allows schedulers to validate multiple version orders for generating a good version order.
Any NWR scheduler with VMVO can validate either a version order based on the all invisible strategy or a version order generated by an underlying scheduler. 
Hereafter, we assume any NWR scheduler adopts VMVO optimization.
If a version order based on the all invisible strategy makes MVSG acyclic, the NWR scheduler with VMVO generates it to improve the performance of write operations.
Otherwise, the NWR scheduler generates the other version order generated by the underlying scheduler.
No matter how many version orders the NWR scheduler with VMVO validates,
it can generate the same MVSG with the underlying scheduler, eventually.
Thus, VMVO yields the same or more commit rate than the commit rate of underlying schedulers.

Furthermore, VMVO allows us to extend conventional schedulers to NWR schedulers easily. 
We have to add the component for validating additional version orders.
However, the implementation cost to extend underlying schedulers is low
because we do not have to modify core modules of them.

VMVO optimization causes the complexity problem because the exhaustive searching problem of version orders is NP-Complete problem \cite{Papadimitriou1982OnVersions,Bernstein1983MultiversionAlgorithms}.
Although schedulers validate multiple version orders for generating good one, the exhaustive search is not practical.
In practice, we adopt validating two version orders; the version order based on the all invisible strategy and the version order generated by underlying schedulers.


==> tex/algorithms.tex <==
\section{Implementation Overview}
\label{sec:implementation_overview}

Next, we show an implementation overview of NWR.
To extend a baseline protocol to a new NWR-extended protocol, we must add followings procedures:

\begin{enumerate}
  \item
         Find and generate an additional version order $\ll^{NWR}$ which satisfies preserving version order rule
  \item
        Collect $successors_j$ and $overwriters_j$ and validate SR-Rule and ST-Rule
\end{enumerate}

Note that we assume these procedures are executed at the time of $t_j$'s commit, and $t_j$ satisfies RC-Rule. 

\subsection{Validating SR-Rule}

When we generate a version order $\ll^{NWR}$ as described above, $\ll^{NWR}$ always satisfies the rules of NWR except for SR-Rule.
Next, we show how to validate SR-Rule.
Let $S, \ll, t_j$ be a triple of a schedule, a version order for the schedule, and a running transaction that satisfies the rules of NWR except for SR-Rule.

To validate SR-Rule, we must check whether some $t_k$ in $successors_j \cup overwriters_j$ has some path into $t_j$ or not.
We separate the validation into two sub-problem.
At first we show how to validate all $t_k$ in $overwriters_J$.
Next, we show for $successors_j$.

\subsubsection{Validating Overwriters}
\label{sec:tracking_overwriters}

In fact, we already have the implementation; the baseline CC algorithm gives us the necessary component.
The definition of $overwriters_j$ indicates a set of $t_k$ such that $t_j \VORW{} t_k$.
It means that a version $x_i \in rs_j$ is an old version, and there exists a newer version $x_k$.
This definition is completely same with \textit{anti-dependency (r-w dependency)} in CSR \cite{Papadimitriou1986TheControl,Hadzilacos1988ASystems} and in Adya's serialization graph \cite{2000:GIL:846219.847380}.
In other words, $t_j$ is anti-dependent (r-w dependent) on $t_k$ if a transaction $t_k$ is in $overwriters_j$.
Fortunately, because the baseline CC algorithm ensures serializability, we always have the implementation of anti-dependency validation.
For example, S2PL \cite{Gray1992TransactionTechniques} guarantees that $overwriters_j = \phi$.
Silo \cite{Tu2013SpeedyDatabases} assumes that $overwriters_j = \phi$ (and aborts $t_j$ if this assumption does not hold).
% only if はない．VOが違うかもしれんし
Therefore, we can reuse the implementation of the baseline CC algorithm for collecting and validating $overwriters_j$.

\subsubsection{Validating Successors}
\label{sec:tracking_successors}

For $successors_j$, the implementation is not simple.
Consider a version order for $S$ which does not include any $x_k$ such that $x_j <_v x_k$ for all $x_j \in ws_j$.
In this case, $successors_j$ is always empty.
In other words, if every $x_j$ for all $x_j \in ws_j$ is the latest version, we do not have to consider SR-Rule validation.
In fact, almost all in-memory CC algorithms choose the latest versions by locking and they do not consider SR-Rule.
Thus, there is no generic and reusable implementations like $overwriters_j$.


\begin{algorithm}[h]
  \begin{algorithmic}
    \Require{$t_j, \ll^{NWR}$}
    \State{$T = \{RN(t_k)| t_k \in successors_j\}$}
    \Comment{(1)} % $collect
    \State %CRLF

    \ForAll{$t_m$ in $T$}
    % w-r
    \ForAll{$y_m$ in $ws_m$}
    \ForAll{$y_n$ in $rs_j$}
    \If{$y_m <_v y_n$ or $y_m = y_n$}
    \Comment{(2) $\WR{}$ to $t_j$} % $t_j \to ..., \WR{} t_j$
    \State %CRLF
    \Return{MVSG is not acyclic}
    \EndIf
    \EndFor
    \EndFor

    \State %CRLF
    % rw
    \ForAll{$y_g$ in $rs_m$}
    \ForAll{$y_j$ in $ws_j$}
    \If{$y_g <_v y_j$}
    \Comment{(3) $\VORW{}$ to $t_j$} % $t_j \to ..., \VORW{} t_j$
    \State %CRLF
    \Return{MVSG is not acyclic}
    \EndIf
    \EndFor
    \EndFor
    \EndFor
    \State{} % CRLF

    \Return{MVSG is acyclic}
  \end{algorithmic}
  \caption{validation of $successors_j$, where $<_v \in \ll^{NWR}$}
  \label{alg:successors_validation_pseudo}
\end{algorithm}

Figure \ref{alg:successors_validation_pseudo} summarizes how our NWR-extended protocols find cyclic paths.
The key point of our method is to focus and find the last edge of cyclic paths.
We validate whether or not the last edge $\to t_j$ exists, for each three type of edges.
In (1), we collect every transaction $t_m$ which is reachable from $t_k \in successors_j$.
Next, (2) and (3) are validations of the acyclicity of MVSG.
Briefly, (2) checks $t_m \to ..., \WR{} t_j$ and (3) checks $t_m \to ..., \VORW{} t_j$.
(2) validates that some $y_n$ in $rs_j$ is newer than $y_m$ in $ws_m$ for some $t_m$.
If it holds, there is a path to $t_j$ from $t_k$ including $\WR{}$ edge, and MVSG is not acyclic.
Likewise, (3) validates that some $y_j$ in $ws_j$ is newer than $y_g$ in $rs_m$ for some $t_m$.
If it holds, there is a path $t_j$ from $t_k$ including $\VORW{}$ edge, and MVSG is not acyclic.
Note that RC-Rule ensures that any transaction $t_m$ does not have a path $t_m \VOWW{} t_j$ because the edge $\VOWW{}$ is added into MVSG only if some transactions read some $x_j \in ws_j$.
Therefore, if we pass validations (2) and (3), and RC-Rule is satisfied, any edge from any $t_k \in successors_j$ cannot reach into $t_j$.

A key observation is that we assume that we have both read-sets and write-sets for all $t_k \in \{successors_j\}$ and for all $t_i \in RN(t_k)$.
This assumption causes huge overhead since it means that transactions must store their read-set and write-set into shared memory.
In the next section, we show that how to store and maintain both read-set and write-set with tiny overhead.


==> tex/future_work.tex <==
\section{Future Work}
The following two problems remain as future work:

\begin{enumerate}
\item Can we find the most efficient way to decide the version order based on the all invisible strategy? For a write operation $w_j(x_j)$, a scheduler based on the all invisible strategy can assign $x_j$ anywhere between $x_0$ and the latest version of $x_{latest}$.
Because different version orders generate different MVSGes, the detail of version orders affects the commit rate.

\item How many version orders should be validated? In addition to the version order based on all invisible strategy, we can sometimes improve the commit rate by validating yet another version order. For example, we can consider the strategy for hot (frequently written) data items; a new version of a hot data item is better to be ordered older to omit, and a new version of a cold data item may be better to be ordered the latest. Because LI-Rule is satisfied only when there exists a concurrent write operation, write operations which access cold items are rarely to be IW operations. Thus, "order some write operations to be old, and order others to be the latest" strategy may work well. However, the best strategy and the best amount of validating version orders depend on workload.
\end{enumerate}

If we know a real workload and access patterns of data items, we may be able to extend a conventional scheduler to an NWR scheduler with validating \textit{better} version orders.


==> tex/lockfreevs.tex <==
\section{Manipulating MergedSet}
\label{sec:lockfreevs}

Next, we show the details of the implementation of LI-Rule and tracking $successors_j$ for a running transaction $T_j$, by using the data structure described in Appendix \ref{sec:implement}.
Briefly, we use FV and Epoch for LI-Rule, and we use MergedRS and MergedWS for SR-Rule.

As described in Appendix \ref{sec:algorithms}, we need to validate that MVSG is acyclic, by using readsets and writesets for all $T_k \in \{successors_j \cup overwriters_j\}$ and all $T_i \in RN(T_k)$.
We compress these sets into MergedRS and MergedWS to manipulate with lock-free fashion.

\begin{algorithm}[t]
  \caption{Tracking of $successors_j$ with MergedRS and MergedWS}
  \label{alg:successors_validation}
\begin{algorithmic}
   \Require{$T_j$}
   
    \ForAll{$x_j$ in $ws_j$}
       \State{MergedRS, MergedWS := Index.get($x$)}
       \Comment{(1)} % $T_j \to ..., \VORW{} T_j$
       
       \State %CRLF
       % w-r
        \ForAll{$vs(y_k)$ in MergedWS}
           \If{$y_i$ $\in rs_j$ and !$(2^4-1 \leq vs(y_k) \land 2^4-1 \leq vs(y_i))$}
             \Comment{(2)} % $T_j \to ..., \WR{} T_j$
             \If{$vs(y_k) \leq vs(y_i)$}
                \State %CRLF
                \Return{MVSG may be not acyclic}
              \EndIf
           \EndIf
         \EndFor
         
         \State %CRLF
         % rw
        \ForAll{$vs(y_k)$ in MergedRS}
           \If{$y_j$ $\in ws_j$ and !$(2^4-1 \leq vs(y_k) \land 2^4-1 \leq vs(y_j))$}
              \Comment{(3)} % $T_j \to ..., \VORW{} T_j$
              \If{$vs(y_k) < vs(y_j)$}
                \State %CRLF
                \Return{MVSG may be not acyclic}
              \EndIf
           \EndIf
         \EndFor
    \EndFor
    \State{} % CRLF

    \Return{MVSG is acyclic}
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:successors_validation} shows the details of Algorithm \ref{alg:successors_validation_pseudo}, which validates that any edge from any $T_k \in successors_j$ cannot reach into a running transaction $T_j$.
We can reduce the number of loop processing than Algorithm \ref{alg:successors_validation_pseudo} by compressing both readset and writeset.
In (1), our NWR schedulers fetch both readset and writeset for all $T_k$ such that $T_k = T_{FV}$ or $T_k \in RN(T_{FV})$ for a transaction $T_{FV}$ which had written $x_{FV}$.
Because whole the data structure is within 128-bits, We can implement fetching MergedRS and MergedWS with lock-free fashion.
In (2) and (3), we treat the counter saturation.
Necessarily, compressing causes the boundary of counters.
Because each slot of MergedRS and MergedWS has only four-bits, if $vs$ returns the number larger than $2^4-1$, we must treat this case as false-positiveness.
Thus, in this case, we have to decide that MVSG may not be acyclic and $T_j$ cannot
commit with the version order based on the all invisible strategy.

\subsection{Updating The Data Structure}

In this subsection, we show how and when the data structure should be updated.
If validations of SR-Rule or LI-Rule for a running transaction $T_j$ with the version order $\ll$ based on the all invisible strategy has failed,
our NWR schedulers validate the other version order $\ll'$ generated by underlying schedulers.
If the validation with $\ll'$ has also failed, NWR schedulers must abort $T_j$.
Otherwise, our NWR schedulers commit $T_j$ with $\ll'$.
In this case, we must update each field of the data structure of $x$ for all $x_j \in ws_j$ and $x_i \in rs_j$.
Updating the data structure leads to improve commit rate with $\ll$ for subsequent transactions.
For example, if LI-Rule is not satisfied with $\ll$, we can update FVes just like $x_{FV} = x_j$ for all $x_j \in ws_j$ and store the current epoch into the epoch field of the data structure.
At the next time, for a new running transaction $T_j'$, our NWR schedulers validate a version order different with $\ll$; if $T_j$ and $T_j'$ access the same data items, all $x_{FV}$ for all $x_j' \in ws_j'$ are updated.
Besides, if $T_j$ and $T_j'$ is in the same epoch, LI-Rule is always satisfied.
Thus, under this policy, we guarantee that validation failures of LI-Rule happen at most only once for each epoch for each data item.

\begin{algorithm}[t]
  \caption{Updating The data structure}
  \label{alg:NWR_updating_ds}
\begin{algorithmic}
   \Require{$T_j$, Index}
   
    \ForAll{$x_j$ in $ws_j$}
       \State{$vs(x_{FV})$, epoch, MergedRS, MergedWS = Index.get($x$)}
       \State %CRLF
       
       \If{$T_j$.epoch $\ne$ epoch}
        \Comment{(1)} % LI-Rule
            \State{$vs(x_{FV})$ := 1}
            \State{epoch := $T_j$.epoch}
            \State{MergedRS := $rs_j$}
            \State{MergedWS := $ws_j$}
            \State % CRLF
       \Else
        \Comment{(2)} % SR-Rule
            \ForAll{$vs(y_k)$ in MergedRS}
                 \If{$vs(y_k) = 0$ or $vs(y_j) < vs(y_k)$}
                     \State{MergedRS[$h(y)$] := $vs(y_j)$}
                 \EndIf
              \EndFor
               \State %CRLF
               
             \ForAll{$vs(y_k)$ in MergedWS}
                 \If{$vs(y_k) = 0$ or $vs(y_j) < vs(y_k)$}
                     \State{MergedWS[$h(y)$] := $vs(y_j)$}
                 \EndIf
              \EndFor
               \State %CRLF
         \EndIf
      \EndFor
      
     \If{$rs_j \ne \phi$}
         \Comment{(3)} % Read
         
         \State{all-older, all-newer = true}
         \ForAll{$x_k$ in $rs_j$}
             \State{$vs(x_i)$ := Index.get($x$)}
              \If{$vs(x_i) < vs(x_k)$}
                  \State{all-newer = false}
              \Else
                   \State{all-older = false}
              \EndIf
           \EndFor

           \If{all-newer or all-older}
              \Return         
              \Comment{(4)} % Optimization
           \EndIf
                      \State %CRLF
           \ForAll{$x_k$ in $rs_j$}
              \State{MergedRS := Index.get($x$)}
                  \ForAll{$vs(y_i)$ in MergedRS}
                      \If{$y_k$ in $rs_j$}
                          \If{$vs(y_i) = 0$ or $vs(y_k) < vs(y_i)$}
                               \State{MergedRS[$h(y)$] := $vs(y_k)$}
                           \EndIf
                       \EndIf
                 \EndFor
           \EndFor
     \EndIf
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:NWR_updating_ds} shows the updating process of the data structure.
Let $\ll, \ll'$ be a version order generated by collecting FVes (based on all invisible strategy) and a version order generated by underlying schedulers, respectively.
Our NWR schedulers process this algorithm only when a running transaction $T_j$ can commit only with $\ll'$.

In (1), we update all FV, epoch, MergedRS, and MergedWS if LI-Rule is not satisfied with $\ll$.
Thus, some $x_{FV}$ for some $x_j \in ws_j$ is written in the old epoch.
Then we update the data structure of each data item $x$ so as to $x_{FV} = x_j$.
In this case, because FV will be updated, MergedRS and MergedWS have to store the information of $T_j$.
Moreover, we rewind the integer $vs$ of the version $x_j$ just like $vs(x_j) = 1$.
Because LI-Rule prohibits schedulers from reordering transactions across epochs, $vs$ only have to reflect the order of versions which have written in the same epoch.
Thus, we can rewind $vs$ safely and prevent counter saturation of MergedRS and MergedWS.

In (2), we must update MergedRS and MergedWS for all $x_j$ in $ws_j$.
We need to update MergedRS and MergedWS for each transaction which is reachable from $T_{FV}$.
Since our scheduler commits $T_j$ with $\ll'$ and $T_{FV}$ is in the same epoch with $T_j$,
there may exist a path such as $T_{FV} \to ... \to T_j$.

In (3), NWR schedulers must update MergedRS for all $r_j(x_k)$ in $op(T_j)$.
Note that we must update MergedRS only when some $T_{FV}$ has some path to $T_j$.
Thus, for reducing the coordination in read-intensive workload,
we optimize the update processing in read operations.
In (4), we check that all $x_{FV}$ is newer or older than $x_k \in rs_j$.
If it holds, we can skip updating MergedRS because $T_j$ will never be included in the cyclic path of MVSG for all subsequent transactions.
Note that $T_j$ is in the cyclic path if and only if there is some path from some $T_{FV}$ to $T_j$, and there is some path to another $T_{FV}$ from $T_j$.
% NOTE これproofない
Moreover, we can implement further optimization based on this consideration; when $T_j$ must update MergedRS, we can retry $T_j$ to read only good versions older or newer than FVes.
Under this optimization, read-only transactions avoid any updating the data structures.

As has been noted, we implement updating the data structure in the lock-free fashion.
Thus, if we need to update some field in the data structure, we must copy it to another location.
After validation and modification, we call atomic operations such as CAS or DCAS to update all field atomically.
When CAS or DCAS has failed, we must retry this algorithm; copy the data structure once more, and retry validation, modification, and calling atomic operations.


==> tex/versionorders.tex <==
\section{Extending Conventional Schedulers To NWR schedulers}
\label{sec:vmvo}

We observed in Section \ref{sec:invisiblewriterule} that NWR schedulers can generate a pair of a schedule and a version order, which includes IW.
In this section, we describe 1) which version order generated by NWR schedulers is useful for improving throughput, and 2) how to extend conventional schedulers to NWR.

\subsection{All Invisible Strategy}
\label{sec:mivo}

To fully optimize write operations, we introduce the \textbf{All Invisible Strategy} for generating version orders.
Let a schedule $S$ and a running transaction $T_j$ such that $c_j, a_j \notin S$.
The version order $\ll$ based on the all invisible strategy satisfies $\forall w_j(x_j) \exists x_k (w_j(x_j) \in op(T_j) \Rightarrow (x_k \in \{x\} \land x_j <_v x_k))$.
That is, all write operations of $T_j$ always become IW operations when schedulers generate $S'$ such that $c_j \in S'$.
By omitting all write operations, the version order based on the all invisible strategy maximizes the performance of write operations.

However, generating the version order based on the all invisible strategy may worse for the performance.
Because MVSGes depend on version orders, commit ratio of schedule depends on version orders.
Thus, if we extend a conventional scheduler to an NWR scheduler, we cannot guarantee that the performance of the NWR scheduler is better or equal to the performance of the underlying scheduler, even in the same workload.

\subsection{Validating Multiple Version Orders}

To keep the commit rate of underlying schedulers and to improve the performance of write operations, we introduce \textbf{Validating Multiple Version Orders (VMVO)}.
In contrast with conventional approaches, maintain and validate the only one version order, VMVO allows schedulers to validate multiple version orders for generating a good version order.
Any NWR scheduler with VMVO can validate either a version order based on the all invisible strategy or a version order generated by an underlying scheduler. 
Hereafter, we assume any NWR scheduler adopts VMVO optimization.
If a version order based on the all invisible strategy makes MVSG acyclic, the NWR scheduler with VMVO generates it to improve the performance of write operations.
Otherwise, the NWR scheduler generates the other version order generated by the underlying scheduler.
No matter how many version orders the NWR scheduler with VMVO validates,
it can generate the same MVSG with the underlying scheduler, eventually.
Thus, VMVO yields the same or more commit rate than the commit rate of underlying schedulers.

Furthermore, VMVO allows us to extend conventional schedulers to NWR schedulers easily. 
We have to add the component for validating additional version orders.
However, the implementation cost to extend underlying schedulers is low
because we do not have to modify core modules of them.

VMVO optimization causes the complexity problem because the exhaustive searching problem of version orders is NP-Complete problem \cite{Papadimitriou1982OnVersions,Bernstein1983MultiversionAlgorithms}.
Although schedulers validate multiple version orders for generating good one, the exhaustive search is not practical.
In practice, we adopt validating two version orders; the version order based on the all invisible strategy and the version order generated by underlying schedulers.

